Globally Convergent Policy Search over Dynamic Filters for Output Estimation

We introduce the first direct policy search algorithm which provably converges to the globally optimal $\textit{dynamic}$ filter for the classical problem of predicting the outputs of a linear dynamical system, given noisy, partial observations. Despite the ubiquity of partial observability in practice, theoretical guarantees for direct policy search algorithms, one of the backbones of modern reinforcement learning, have proven difficult to achieve. This is primarily due to the degeneracies which arise when optimizing over filters that maintain internal state. In this paper, we provide a new perspective on this challenging problem based on the notion of $\textit{informativity}$, which intuitively requires that all components of a filter's internal state are representative of the true state of the underlying dynamical system. We show that informativity overcomes the aforementioned degeneracy. Specifically, we propose a $\textit{regularizer}$ which explicitly enforces informativity, and establish that gradient descent on this regularized objective - combined with a ``reconditioning step'' - converges to the globally optimal cost a $\mathcal{O}(1/T)$ rate. Our analysis relies on several new results which may be of independent interest, including a new framework for analyzing non-convex gradient descent via convex reformulation, and novel bounds on the solution to linear Lyapunov equations in terms of (our quantitative measure of) informativity.

==> body/analysis_overview.tex <==
%!TEX root = ../main.tex



In this section, we highlight the key features of the proof of our main result, \Cref{thm:main_rate}, and in doing so, illustrate the benefits of the differentiable convex liftings framework. At a high level, the proof is based on showing that, as long as the iterates $\sfK_s$, suitably normalized, remain in the set of informative filters $\calKexp$, the regularized objective, $\cL_{\lambda}$ is smooth and satisfies a gradient dominance condition. Having established these two properties, an elementary analysis of gradient descent gives the desired convergence rate. 

The bulk of the analysis lies in using the \DCL{} framework to prove the gradient dominance or weak-PL condition and arguing that the $\cL_{\lambda}$ objective is sufficiently smooth and Lipschitz by analyzing the solutions to various Lyapunov equations. We structure this section as per the above discussion. First, we prove an abstract convergence guarantee showing how gradient descent converges at a $\cO(1/T)$ rate on any function $f$ that satisfies the regularity conditions described above. Then, we prove that if an optimization problem has a differentiable convex lifting, then the underlying objective must satisfy the weak-Polyak-{\L}ojasiewicz (PL) (i.e. gradient domination) 
%\kzcomment{first time PL appears? re-define it!} 
property. We conclude analysis by illustrating how the regularized $\OE$ problem admits a \DCL{} and verifying the requisite smoothness and Lipschitz conditions.  

\paragraph{Preliminaries.} Before moving on, we introduce some of the necessary notation and definitions. To neatly accommodate optimization over constrained domains,  we express functions $f: \R^d \to \Rebar$ as taking values in the extended reals $\Rebar := \R \cup \{\infty\}$.\footnote{Because we solely consider minimizations, $\Rebar$ does not include $-\infty$} 
We denote the domain of these functions, $\dom(f): \{x:f(\cvxarg)\ne \infty\}$, as the set of all points for which $f$ is finite and say $f$ is proper if $\dom(f) \ne \emptyset$. 
We define their minimum values by $\inf(f) = \inf_{\bx \in \R^d} f(\bx)$ and define the domain of suboptimal points as $\dom_{>}(f) := \{\bx \in \dom(f): f(\bx) > \inf(f)\}$. All functions are assumed to take extended real values, and are infinite outside their domain when not otherwise defined (for example, in the case of an ill-posed inverse).
Lastly, given $\calK \subset \R^d$, we say that $f \in \Cclass^k(\calK)$ if it is $k$-times continuously differentiable on some open set containing $\calK$. 
%When defined, we let $\nabla f(\bx) \in \R^d$ denotes the gradient and $\nablatwo f(\bx) \in \R^{d \times d}$ denote the Hessian of $f$ at $\bx$. We say that $\bx$ is a first-order critical point of $f$ if $f \in \Cclass^1(\{\bx\})$ and $\nabla f(\bx) = 0$.%, and a second-order local minimum if $f \in \Cclass^2(\{\bx\})$, $\nabla f(\bx) = 0$ and, in addition, $\nablatwo f(\bx) \succ 0$. \mscomment{i defined this so we could see if there are local minima in this sense}
%\begin{remark}[Constraints via Extended-Real Functions] Let $f:\calK \subset \R$ be a function defined only on some set $\calK \to \R^d$. We can represent $f$ as an extended real function defined on all of $\R^d$ by defining $f(\farg) = \infty$ for all $x \in \R^d \setminus \calK$. In this manner, extend-real functions can encode arbitrary constraint sets $\calK$. 
%\end{remark}
\paragraph{Key regularity conditions.} We now state the two key properties of $f$ which guide our analysis. 
\begin{definition}[Regularity on $f$]\label{defn:reg} Given a set $\calK \subset \R^{d}$ and proper $f:\R^{d} \to \Rebar$, we say that
\begin{enumerate}
	\item $f$ satisifes $\alpha$-weak PL on $\calK$ if $f \in \ccone(\calK)$ and $\|\nabla f(\farg)\| \ge \alpha (f(\farg) - \inf(f)$, for some $\alpha > 0$.\footnote{Again, $\inf(f)$ is the infimum   over $\R^d$. Since  $f$ is proper, $\inf(f) > -\infty$.}
	\item $f$ is $\beta$-upper-smooth on $\calK$ if $f \in \cctwo(\calK)$ and for all $\farg \in \calK$, $\nablatwo f(\farg) \preceq \beta \bI$.
\end{enumerate}
\end{definition}
The purpose of smoothness is to ensure gradient descent finds approximate stationary points. It is a local condition in that it depends only on the properties of derivatives. Weak-PL,  on  the other hand, is a \emph{global condition}: it depends both on the value of $f$ and magnitude of its gradient, \emph{as well as the global minimum value of $f$}. Note that weak-PL implies that there are no suboptimal stationary points, and further bounds the suboptimality of approximate stationary points. 

%Note that while smoothness is a local condition in the sense that it need only hold for points in $\calK$, weak-PL is a global condition in that it relates points in $\calK$ to the global minimize of $f$. 
%The most powerful consequence of the weak-PL property is \emph{all first-order critical points of $f$ on $\calK$ are global minima.}
%In \Cref{sec:DCL}, we argue that the existence of a (suitably formulated) convex reparametrization of $f$ implies the $\alpha$-weak-PL property, which can be thought of a strengthening of \Cref{fact:no_suboptimal_sp}. Combined with smoothness, the weak-PL property provides sufficient conditions for gradient-descent to converge to a global minimum; see \Cref{sec:optimization_reco} for details 

\begin{comment}
; we state an informal version of this result, and defer a more exact statement (with additional bells-and-whistles) to 
\begin{lemma}[Informal] Let $f$ be an extended-real function, $\farg_0 \in \dom(f)$, and let $\calK$ be the level set $\{\farg: f(\farg) \le f(\farg_0)\}$. Then, if $f$ is $\alpha$-PL and $\beta$-upper-smooth on $\calK$, $T$-iterations of gradient descent on with approximate step size produces an $\farg_T$ with 
\begin{align*}
f(\farg_T) - \inf(f) \le \left(f(\farg_0) - \inf(f)\right) \cdot \BigOh{\frac{\beta}{\alpha^2 T}}. 
\end{align*}
\end{lemma}
Observe that while $\beta$-upper-smoothness is a local property of $f$, $\alpha$-weak-PL pertains to its \emph{global} structure, and hence considerably more challenging to verify. The following section introduces a new framework to verify this condition. 
\end{comment}



\subsection{Optimization with a reconditioning step}\label{sec:optimization_reco}
As discussed previously, we now illustrate how the previous two conditions suffice to show a convergence result for a variant of gradient descent that includes a ``reconditioning step'' at every iteration. 
\begin{definition}[Reconditioning operator]\label{defn:reco} Given $f: \R^d \to \Rebar$, we say that $\bLambda: \dom(f) \to  \psd{n}$ is a reconditioning operator for $f$ if for every $\farg \in \dom(f)$ such that $\bLambda(\farg) \succ 0$, there exists an $\farg' \in \dom(f)$ such that $\bLambda(\farg') = \eye_{n}$ and $f(\farg') = f(\farg)$. We define the set $\recond_{\bLambda}(\bx) := \{\farg': f(\farg') = f(\farg), \quad \bLambda(\bx) = \eye_n\}$ as the set of such points. We say $\farg$ is reconditioned if $\bLambda(\farg) = \eye_n$.
\end{definition}

This reconditioning generalizes the reconditioning  step in $\algname$ where we choose $\bLambda(\sfK) = \bSigma_{\sfK,22}$ and where reconditioning is achieved by a similarity transformation of $\sfK$ (recall \Cref{sec:algorithm}). Reconditioning serves to ensure that $f$ need only be well-behaved (i.e. satisfy upper-smoothness and weak-PL for suitable constants) on a restricted set of approximately reconditioned parameters $\farg: \bLambda(\farg) \approx \eye_n$. The following proposition is the guiding template for the overall convergence analysis.

\begin{proposition}\label{prop:reco_descent} Let $f:\R^d \to \Rebar$, $\farg_0 \in \dom(f)$, and let $\bLambda$ be a reconditioning operator for $f$ such that $\bLambda(\farg_0) \succ 0$. Define the reconditioned level set,
\begin{align*}
\calK(\farg_0) := \left\{\farg \in \R^d: f(\farg) \le f(\farg_0) \,\text{ and  }\, \|\bLambda(\farg)- \eye_n\|_{\op} \le \frac{1}{2}\right\}.
\end{align*}
Assume that the function $\farg \mapsto \bLambda(\farg)$ is $\LrecoK$-Lipschitz as a mapping from $(\R^d,\|\cdot\|) \to (\psd{n},\|\cdot\|_{\op})$ and that $f$ is $\betaK$-upper-smooth, $\LfK$-Lipschitz, and satisfies the $\alphaK$-weak PL condition for points in $\calK(\farg_0)$. Lastly, let $\{ \eta_k\}_{k=0}^\infty$ be a series of step sizes such that $\sup_k \eta_k \le \min\{\frac{1}{\betaK},\frac{1}{2\LfK\LrecoK}\}$. If iterates are chosen according to, 
\begin{align}
\tilde\farg_k \in \recond_{\bLambda}(\farg_k), \quad \farg_{k+1}  = \tilde \farg_k - \eta_k\nabla f(\tilde \farg_k) \label{eq:reco_updates},
\end{align}
then for all $k \geq 1$ it holds that
\begin{align}
f(\farg_{k})\le  \frac{2}{\alphaK^2 \eta} \cdot \frac{1}{k}, \quad \text{ where } \eta := \min_{k \ge 1}\eta_k. \label{eq:guaranteed_reco_descent}
\end{align}
\end{proposition}

Relative to standard analysis of gradient descent, the above guarantee \Cref{eq:guaranteed_reco_descent} may seem strange in that there is no explicit dependence on the initial iterate $\farg_0$. However, the PL-constant $\alpha$ typically scales proportionally to the inverse of a Euclidean distant $\|\farg_0 - \farg_\star\|$, where $\farg_\star$ minimizes $f$ (this is true, for example, in convex functions). In this case, we recover the familiar scaling for smooth convex optimization,  $f(\farg_{k}) - \inf(f)\lesssim  \frac{2 \|\farg_0 - \farg_\star\|^2}{\eta k }$. Furthermore, note that, in our setting the maximal step size may, and in fact does, also depend on $\calK$ through the Lipschitz constants. 
\begin{remark}[Implementation via line search] \mscomment{to fill in}
\end{remark}


%Now, we move onto to proving that if we perform direct policy search as per \algname, then the regularized $\Loe$ objective will satisfy all the regularity conditions necessary to apply \Cref{prop:reco_descent}.

\subsection{Weak PL via the \DCL{} framework}\label{sec:DCL}

Next, we provide a generic recipe for verifying the weak-PL condition (required by \Cref{prop:reco_descent} above), which ensures that approximate stationary points of $f$ are approximate minimizers of $f$. We call this recipe a \emph{differentiable convex lifting}, or \DCL. As discussed in the introduction, to prove rigorous convergence results,  our notion of a convex reparameterization, or \DCL{}, needs to be considerably more flexible than that described in \Cref{ass:convex_reform_simple}. 

\begin{restatable}{definition}{dcldef}\label{defn:DCL} A triplet of functions $\dcltriple$ forms a \DCL{} of a proper function $f: \R^{\dfarg} \to \Rebar$ if
\begin{enumerate}
\item $\fcvx: \R^{\dcvx} \to \Rebar$ is an (extended-real valued) convex function whose minimum is attained by some $\cvxargst$, $\fcvx(\cvxargst) = \inf(\fcvx) > - \infty$.
\item For some additional number of parameters $\dxi \ge 0$, $\flift: \R^{\dfarg +\dxi} \to \Rebar$ is related to $f$ via partial minimization: $f(\farg) = \min_{\xiarg \in \R^{d_{\xi}}} \flift(\farg,\xiarg)$. 
\item For an open set $\tilset $ containing $\dom(\flift)$, $\Phi: \tilset \to \dom(\fcvx)$, is $\ccone(\tilset)$, and relates $\flift$ to $\fcvx$ via $\flift(\cdot) = \fcvx(\Phi(\cdot))$. 
\end{enumerate}
\end{restatable}


 Intuitively, a \DCL{} of a function $f$ is composed of a triplet of functions $\dcltriple$ where $\fcvx$ is the convex reparameterization on $f$. However, rather than relating $f$ directly to $\fcvx$, we ``lift'' $f$ to a function $\flift$ by appending auxiliary   variables. We then let $\Phi$ describe the reparametrization which maps the domain of $\flift$ to that of $\fcvx$ in this higher dimensional space. To avoid degeneracies in the landscape and guarantee that gradient domination  holds, the key property of \DCL{}s is that the rank of the derivative of $\Phi$ must be as least as large as the dimension of the domain of the convex function $\fcvx$. This guarantees that any desired  perturbation of the parameters of $\fcvx$ can be achieved by suitably perturbing the parameters of $\flift$, and applying $\Phi$. Compared to directly reparametrizing $f$, including $\flift$ in the definition adds additional columns to $\nabla\, \Phi$ thereby making the rank condition easier to meet. 
 
% We would like to emphasize that the original

The mere existence of a \DCL{} guarantees that the original, possibly nonconvex function $f$ has no suboptimal stationary points. We view the following result as the operationalized version of \Cref{fact:no_suboptimal_sp} for \DCL{}s.

\begin{theorem}[Weak gradient domination for \DCL{}]\label{thm:DCL} Let $f: \R^{\dfarg} \to \Rebar$ be a proper function with \DCL{} $\dcltriple$. Then, for any $\farg \in \domsub(f)$ at which $f$ is differentiable, $f$ satisfies the weak-PL condition:
%\kzcomment{do we know the max in the definition of $\alpha_{\DCL{}}$ over $\xiarg$ can be achieved? shall we use $\sup$?}
\begin{align}
\|\nabla f(\farg)\| \ge \alphadcl(\farg) \cdot\left(f(\farg) - \inf(f)\right), \quad \text{ where } \alphadcl(\farg) := \max_{\substack{\cvxargst \in \argmin \fcvx(\cdot) \\ \xiarg \in \argmin \flift(\farg,\cdot)}}  \frac{\sigma_{\dcvx}(\nabla \,\Phi(\farg,\xiarg))}{ \|\Phi(\farg,\xiarg) - \cvxargst\| } \label{eq:alpha_theta}.
\end{align}
\end{theorem}
The PL-constant $\alphadcl(\farg)$ depends on two quantities. Letting $\xiarg$ be the auxiliary variable such that $f(\farg) = \min_{\xiarg \in \R^{d_{\xi}}}\flift(\farg,\xiarg)$, the numerator is the $d_z$-th singular value of $\nabla \Phi(\cdot)$ evaluated at $(\farg,\xiarg)$. As described previously, this captures how large perturbations of $\flift$'s arguments must be in order to achieve a desired perturbation of the arguments of $\fcvx$, under the reparameterization $\Phi$. The definition of a \DCL{} further rules out ``trivial reparametrizations'' which might seem to skirt the dependence on $\sigma_{d_z}(\nabla \Phi)$; see \Cref{rem:trivial_par} in the Appendix for details. On the other hand, the denominator measures the Euclidean distance between any minimizer of the convex function $\fcvx(\cdot)$ and image of $(\farg,\xiarg)$ under the reparameterization $\Phi$, and can be bounded under quite benign conditions. Importantly, while \Cref{thm:DCL} does require differentiability of $f$ and $\Phi$, it \emph{does not} impose any smoothness restrictions on $\flift$ or $\fcvx$. In particular, $\fcvx$ can be highly non-smooth and, due to the extended-real function formulation, can also include constraints. 

\begin{proof}[Proof sketch of \Cref{thm:DCL}] Although the formal proof requires special care to handle the extended-real valued formulation that allow $\flift$ and $\fcvx$ to be finite only on restricted domains, and possible non-smoothness, the main ideas behind the result are quite simple.  

Since $\fcvx$ is convex, the suboptimality of a point $\farg$ is bounded by $\norm{\grad \fcvx(\farg)}$. Using the \DCL{} definition and analyzing the inverse image of a point under $\Phi$, we can also establish a gradient domination  result for $\flift$. Lastly, we can establish a weak-PL result for the original function $f$ by observing that,  since $f$ is related to $\flift$ by partial minimization, the gradients of $f$ must always be larger than those of $\flift$.
%First, some notation: given $\farg \in \dom(f)$, let $\xiarg$ be such that $f(\farg) = \flift(\farg,\xiarg)$, and let $\tilarg = (\farg,\xiarg)$, $\cvxarg = \Phi(\tilarg)$, and $\cvxargst \in \argmin (\fcvx)$; further, assume $\farg$. Since $\fcvx$ is convex (and assuming differntiability), the subgradient inequality gives $\fcvx(\cvxarg) - \fcvx(\cvxargst) \le \langle \nabla \fcvx(\cvxarg), \cvxarg - \cvxargst \rangle$. % Applying the change of variables $\Phi$, and noting that $\fcvx(\cvxarg) - \fcvx(\cvxargst) = f(\farg) - \inf(f)$, we have $f(\farg) - \inf(f) \le \langle \nabla \flift(\tilarg), \nabla \cvxarg - \cvxargst \rangle$
\end{proof}



==> body/new_intro.tex <==
%!TEX root = ../main.tex

\renewcommand{\OE}{{\normalfont \texttt{OE}}}
\newcommand{\DCL}{{\normalfont\texttt{DCL}}}

\section{Introduction}

Data used for prediction and control of real world dynamical systems is almost always noisy and imperfect. 
Seeing how sensors and other measurement procedures inevitably introduce errors into the available datasets, designing reliable learning algorithms for these noisy or partially observed domains requires confronting fundamental questions of disturbance filtering and state estimation. 
Despite the ubiquity of partial observation in practice, these concerns are often neglected in more traditional analysis of learning and control that assume perfect observations of the underlying dynamics. 

In this work, we study the output estimation (OE) problem or learning to predict in partially observed linear dynamical systems. 
The output estimation problem is one of the most basic problems in theoretical statistics and learning theory. Furthermore, its solutions have been successfully applied in a wide variety of domains from control theory to biology and economics. 
We revisit this classical problem from a modern optimization perspective, and study the possibilities of learning the optimal predictor via model-free procedures and direct policy search.

Relative to more traditional model-based procedures, which directly estimate the underlying dynamics and then return a solution by solving a convex optimization problem offline, model-free methods offer several promising advantages. 
First, direct policy search often yields controllers that are substantially simpler than the dynamics they influence. For example, the vast majority of industrial control systems are built upon proportional-integral- derivative (PID) methods. These optimize three scalar variables, yet successfully regulate complex, high-dimensional systems (e.g chemical plants). 
Furthermore, from a robustness perspective, whenever there is uncertainty in the underlying dynamics, model-based approaches require the designer to pre-specify a structured uncertainty set and to optimize a worst-case objective over the predefined set of models. 
Conversely, direct policy search using gradient descent can directly operate using information from the true system, rather than an inaccurate or contrived approximation.

In light of these advantages, there has recently been significant interest from both theoreticians and practitioners in understanding the foundations of model-free control. 
However, so far, this attention has been mostly focused on problems with full-state observation such as the linear quadratic regulator (LQR) or fully-observed Markov Decision Processes (MDPs). 
Progress in dealing with partially observed problems has thus far proven to be quite challenging due to the difficulties associated with summarizing the past history of observations and optimizing over dynamic policies that maintain internal state. 
In this paper, we provide the first policy search algorithm which provably converges to the globally optimal filter for the OE problem and shed new light on the intricacies of the underlying optimization landscape.   

%We now review the formal problem setup and introduce our contributions in more detail:



\paragraph{The Output Estimation problem.} We study one of the simplest and most basic problems with partial observability: the  \emph{output estimation} (\OE) problem.
%A detailed problem specification is given in SECTION; 
In brief, the goal is to search for a predictor of the output $\po(t)$ of a linear dynamical system given partial measurements $\mo(t)$. 
%by directly running gradient descent over a particular objective. 
For the \emph{true system} with states $\sx(t)$ and dynamics that evolve according to,
\begin{equation}\label{eq:true_system}
\begin{aligned}
&\tfrac{\rmd}{\rmd t} \sx(t) = \sA\sx(t) + \sw(t), \quad \sy(t)=\sC\sx(t) + \sv(t), \quad \po(t) = \sO \sx(t), \quad \sx(0) = 0, \\
&\quad \sw(t) \iidsim \calN(0,\sW), \quad \sv(t) \iidsim \calN(0,\sV),
\end{aligned}
\end{equation}
the goal is to find the parameters $\fparams = (\fA,\fB,\fC)$ of the \emph{filter} (interchangably, \emph{policy}),
\begin{equation}\label{eq:filter_system}
\tfrac{\rmd}{\rmd t} \fx(t) = \fA\fx(t) + \fB\sy(t), \quad \fo(t) = \fC\fx(t),
\end{equation}
that minimizes the steady-state prediction error,
\begin{align}\label{eq:loe}
\mathcal{L}_{\OE}(\fparams) := \lim_{T \to \infty} \frac{1}{T}\left(\mathbb{E} \int_{0}^{T} \| \po(t) - \fo(t) \|^2 \rmd t\right) = \lim_{t \to \infty} \mathbb{E} \| \po(t) - \fo(t) \|^2.
\end{align}
In this paper, 
we study solving the \OE\ problem via model-free methods, where the goal is to search for the optimal filter parameters $\fparams = (\fA,\fB,\fC)$ using direct policy search
%the optimization of $\mathcal{L}_{\OE}(\fparams)$ via gradient descent, 
%with decision variables corresponding to the filter parameters ,
without knowledge or estimation of the true system parameters $\sA, \sC, \sO, \sW, \sV$;
cf. \Cref{sec:prelim} for a detailed problem description. 

While the \OE\ problem is not a control problem per se, it is an attractive stepping stone for studying model-free control. 
It is a special case of the partially observed linear quadratic regulator problem (\LQG).
In fact, it is one of the two subproblems solved to obtain the solution to \LQG\ via the separation principle \citep{aastrom1971introduction,dgkf89}. 
%and played an important role in the development of state-space solutions to \LQG CITE[DGKF]. 
Furthermore, like \LQG, optimal policies for the \OE\ problem are \emph{dynamic}, in the sense that they maintain an internal state. 
It therefore serves as a valuable testbed  to develop the theoretical foundations of direct policy search for this important class of policies which has thus far remained poorly understood.
Finally, 
%and perhaps most importantly, 
\OE\ is an important problem in its own right. Both in theory and in practice, advances in predicting partially observed linear systems have led to widespread successes in a variety of areas from controls, to biology and economics,
cf., e.g.  \cite{athans1974importance}.
\subsection{Contributions}\label{ssec:contributions}

In this paper, we demonstrate that running gradient descent on the $\mathcal{L}_{\OE}$ objective routinely fails to recover an optimal filter, 
and propose a novel policy search method 
%with a slightly more model-based flavor 
which \emph{provably converges to a globally optimal solution}. 
 
A key concept underpinning our results is a property we refer to as \emph{informativity},
which requires each component of the policy's internal state $\fx$ to capture
some information about the state $\sx$ of the true system.
More precisely, a policy is said to be \emph{informative}
if the steady-state correlation matrix 
$\bSigma_{12} := \lim_{T \to \infty} \frac{1}{T}[\int_{0}^T\sx(t)\fx(t)^\top \rmd t]$
is full-rank.\footnote{For simplicity, we assume knowledge of the \emph{dimension} of the true system state, and parameterized are policies so that $\sx$ and $\fx$ are of the same dimension.}  
%\kzcomment{reminder: later we might make this point sound less ``necessary'' (given the latest empirical result?)?}
Our contributions are summarized as follows:


\begin{itemize}
	\item \textbf{Limitations of direct policy search.} 
	Through both simulations and mathematical counterexamples,  we show that  gradient descent on the prediction loss $\Loe(\cdot)$ \emph{routinely fails} to recover the optimal filter for $\OE$ problem. 
%	This finding corroborates prior work on the related \LQG{} problem \mscomment{cite}. 
	This finding is consistent with {(but not a direct consequence of)} prior work on the \LQG\ problem by \cite{tang2021analysis}. %, of which \OE\ is a special case.
%	Nevertheless, \emph{the failure of gradient descent is surprising, because the $\Loe$ policy search objective admits  convex reparametrization}, (see \Cref{sec:techniques}), on which one might expect gradient descent to be effective.
	Nevertheless, the failure of gradient descent on \OE\ (and \LQG) remains puzzling, as both can be reformulated as convex programs \citep{scherer97lmi}, a fact which at first glance seems to rule out suboptimal 
	stationary points in the policy search space, cf. \Cref{sec:techniques}.

	\item 

	\textbf{Structure of the \OE\ optimization landscape.} 
	We reconcile this apparent contradiction - the existence of convex reformulations and the failure of policy search - by studying cases in which
%	these convex reformulations 
	the former
	breaks down. 
	We show that suboptimal stationary points can arise when the internal state $\fx$ of the filter is non-informative  about the state $\sx$ of the true system, in the sense described above. 
	%\kzcomment{loved this one!  but still, do we need to mirror/connect to lina's result here, too? since they have also reconciled by claiming that ``suboptimal stationary points can arise when XXXX'', where ``XXXX'' there is non-minimality of the controller. Or, we emphasize \OE\   by starting with  ``For \OE\  problem, we show that...'' (no need to mention them here anymore)?} 
	These are precisely the points at which certain mappings comprising the convex reformulation are no longer well-defined.  
	We also establish the converse: 
	when $\fx$ is ``uniformly informative'' about $\sx$, all stationary points are globally optimal. 

	
	\item \textbf{A provably convergent policy search algorithm.} 
	Building on this insight, 
	we propose a regularizer $\cR$ that ensures the
	internal state of the learned policy remains  ``uniformly informative'' about the state of the true system.
	Moreover, 
	we prove that gradient descent on the {\it regularized} objective $\Loe(\cdot) + \lambda \cR(\cdot)$ converges at a $\BigOh{1/T}$ rate to an optimal policy. 
	

	\item \mscomment{Simulation on Nonlinear system?}
\end{itemize}
On the way to establishing these results, we introduce a number of analytic and algorithmic techniques, which we believe may be useful for later work. 


\subsection{Our Techniques}\label{sec:techniques}


\paragraph{Convex reformulations.} 
Our approach is centered around the idea of {\emph{convex reformulations} of control synthesis problems,} which are by now well known within the controls literature  \citep{scherer97lmi}, and the following fact regarding functions which admit these reformulations.

%Roughly speaking, a smooth change of variables that makes the cost function convex (in the new variables),
%rules out the possibility of any suboptimal stationary points in original nonconvex function. 
%We can formalize this statement as follows.

%Consider a differentiable and possibly \emph{nonconvex} function
%$\jf:\R^{\jnx}\mapsto \R$ which is to be minimized over $\R^\jnx$.
%Further, assume that $\jf_\opt \defeq \min_\jx \ \jf(\jx)$ is finite. 
\begin{assumption}[Convex reformulation]\label{ass:convex_reform_simple}
	Let $\jf:\R^{\jnx}\mapsto \R$  be a differentiable, possibly nonconvex function such that $\min_\jx \ \jf(\jx)$ is finite. There exists a differentiable function $\jch:\R^\jnn\mapsto\R^\jnx$ satisfying the following two properties:
	(i) the mapping $\jch$ is surjective\ie for all $\jx\in\R^\jnx$ there exists $\jn\in\R^\jnn$ such that $\jx=\jch(\jn)$,
	(ii) under the change of variables the function $\jh(\jn)\defeq\jf(\jch(\jn))$ is differentiable and \emph{convex}.
\end{assumption}


\begin{restatable}{fact}{cvxfact}\label{fact:no_suboptimal_sp}
If a function $f$ satisfies \cref{ass:convex_reform_simple},
then all first-order stationary points, $\jx$ s.t $\grad \jf(
\jx)=0$, are globally optimal.	
\end{restatable}




The \OE{} problem, \LQG{}, and many other related control tasks admit convex reformulations in the spirit of \cref{ass:convex_reform_simple}. 
Given that gradient descent (under some additional mild regularity assumptions) converges to stationary points, we might hope that \cref{fact:no_suboptimal_sp} guarantees that direct policy search on the \OE{} filter will succeed at finding an optimal policy, when applied to loss functions admitting such convex reformulations. 

Somewhat surprisingly, we find that this is emphatically not the case: 
gradient descent on the $\Loe$ objective routinely converges to suboptimal solutions.\footnote{As noted above, failure modes for the \LQG{} problem were presented by \cite{tang2021analysis}. } 
While \cref{fact:no_suboptimal_sp} is attractive for its simplicity and broad applicability, 
a number of additional technical hurdles must be surmounted before
it can be used to draw 
%one can arrive at 
positive conclusions
about
%concerning 
the behavior of gradient descent. 
We now discuss these in further detail.
%
%a simple consequence of the fact that, 
%by the chain rule for differentiation, 
%we have $\grad \jh (\jn) = \grad \jf (\jx) |_{\jx=\jch(\jn)} \cdot \grad \jch(\jn)$,
%and so any stationary point $\jx'$ of $\jf(\jx)$ must also show up as a stationary point $\jn'$ of $\jh(\jn)$, with $\jx'=\jch(\jn')$.
%However, $\jh(\jn)$ cannot have any such stationary points that are suboptimal, as $\jh(\jn)$ is convex.
%A complete proof is provided in \jucomment{some appendix}. 

\paragraph{Loss of informativity: A pitfall for convex reformulation.}%\kzcomment{or ``Degenerate Parameterizations''?} 

The key shortcoming of applying \Cref{fact:no_suboptimal_sp} to the output estimation problem is hidden in the surjectivity assumption. 
There may be many filters $\fparams$ with finite cost $\Loe(\fparams)$, 
which are not in the image of the reformulation map $\jch(\cdot)$. 
The existence of a convex reformulation has nothing to say about the suboptimality of such points, and hence the conclusion of \cref{fact:no_suboptimal_sp} does not apply.
In fact, suboptimal stationary points can indeed arise at such points in the optimization landscape.\footnote{Not all stationary points that are not in the image of $\jch(\cdot)$ are suboptimal, cf. \cref{asm:ctrb_of_opt} and \cref{app:ctrb_assumption}.} The ``degenerate'' regions in which the convex reformulation breaks down are precisely those where \emph{informativity}, in the sense defined in \Cref{ssec:contributions}, breaks down. Conversely, for all $\fparams$ for which $\bSigma_{12}$ is full-rank, $\jch(\cdot)$ is surjective,   and the optimality of first-order stationary points holds. 
\paragraph{Regularization for informativity.}
In light of the above observation, one might hope to restrict the search to filters for which $\bSigma_{12}$ is full rank\ie filters with internal state that is \emph{informative}. 
For example, in the spirit of barrier methods, we might find a regularizer $\cR(\fparams)$ which enforces $\sigma_{\min}(\bSigma_{12}) > 0$ whenever $\cR(\fparams)$ is finite. However, regularization is often known to {\it bias} the solution to the regularized problem, such that $\Loe(\cdot)$ and $\Loe(\cdot) + \lambda \cR(\cdot)$ have different global minima. Furthermore, \Cref{fact:no_suboptimal_sp} sheds little light on how much regularization affects the quality of the solution. Similar pitfalls can also arise with hard constraint formulations. 
Fortunately, we show that \OE\ admits a regularizer $\cR(\cdot)$ for which: 
(i) all global minimizers of $\cR(\cdot)$ are \emph{also global minimizers of} $\Loe(\cdot)$, and 
(ii) roughly speaking, there exists a common mapping $\jch$ such that both $\cR(\jch(\cdot))$ and $\Loe(\jch(\cdot))$ are convex. 
Hence, $\Loe(\cdot) + \lambda \cR(\cdot) $ admits a convex reformulation, and $\jch$ is surjective onto the set of filters $\fparams$ for which $ \Loe(\fparams) + \lambda \cR(\fparams)$ is finite. 
As a result, the conclusion of \Cref{fact:no_suboptimal_sp} holds, and all stationary points of the regularized objective are globally optimal. 

\paragraph{An operationalized analysis of convex reformulations.} 
Beyond this problem of loss of informativity,
%\kzcomment{or ``degenerate representation (currently used)/parameterization (which I think might make more sense)''? but either way, I am not sure if it is accurate to say ``degenerate filters''.}, 
there are a number of additional obstacles standing between the existence of a convex reformulation and the success of direct policy search. 
For one, \Cref{fact:no_suboptimal_sp}  does not address the suboptimality of \emph{approximate} stationary points. 
Second, while $ \Loe(\cdot) + \lambda \cR(\cdot)$ admits a convex reformulation $\jh(\cdot)$, there can be values at which $\jch(\cdot)$ and $\jh(\cdot)$ may not be differentiable. 
Lastly, as per our earlier discussion, both the cost $ \Loe(\cdot) + \lambda \cR(\cdot)$ and its convex reformulation have a restricted domain on which they take finite values, while, \Cref{fact:no_suboptimal_sp}  assumes an {\it unconstrained}  domain \ie $\jx\in\R^\jnx$.

To address these three 
%limitations\kzcomment{are they all ``limitations''?}, 
challenges, 
we introduce a new framework for convex reparametrization which we call \emph{differentiable convex liftings} (\DCL ), which accommodates both constraints and the non-differentiability of $\jh(\cdot)$. 
Informally, a \DCL{} ``lifts'' the nonconvex $f$ to a function $\flift$ with $n_y \ge n_x$ parameters, which may also be nonconvex, but need not be differentiable.
Furthermore, $\flift$ may take values in the extended reals, to incorporate constraints.
A \DCL{} establishes approximate optimality of approximate stationary points, provided there exists a map $\Phi$ and a convex function $\jh$ with $n_{\nu} \le n_y$ parameters such that $\flift(\cdot) := \jh(\Phi(\cdot))$. 
Intuitively, $\Phi$ corresponds to the inverse of the map $\Psi$ in \Cref{ass:convex_reform_simple}, though this parameterization allows more flexibility because $n_y > n_{\nu}$ may be permitted. 
For such liftings, we show the following result which we view as a strengthened, operationalized version of \Cref{fact:no_suboptimal_sp}:
\begin{theorem}[Informal]\label{thm:informal_dcl}
Let $\jf$ be a {smooth} nonconvex function which admits a \emph{differentiable convex lifting} $(\flift, \jh,\Phi)$ such that $\sigma_{d_z}(\nabla \Phi(\cdot))$ is bounded away from zero. 
If $\jh(\Phi(\cdot))$ has compact level sets, then any $\jx$ such that $\|\nabla \jf(\x)\|_2 \le \epsilon$, satisfies $\jf(\jx) - f_{\star} \le \BigOh{\epsilon}$.  Here, $\flift$ and $\jh$ need not be differentiable, and may only be defined (or finite) on restricted, and possibly nonconvex domains. 
%\kzcomment{do we really need the last sentence?}\mscomment{I like this, its one of the most important things about the result. }
\end{theorem}

\paragraph{Policies  with well-conditioned internal state covariance.} A necessary condition for informativity is that the internal state covariance $\bSigma_{22} = \lim_{t \to \infty}\Exp[\fx(t)\fx(t)^\top]$ is strictly positive definite. We find it necessary to ensure that $\bSigma_{22}$ is well conditioned in order to guarantee that the conditions of \Cref{thm:informal_dcl} (smoothness of $\jf$, conditioning of $\nabla\, \Phi$, and compact level sets) hold. To this end, we augment gradient descent on the regularized objective $\Loe(\cdot) + \lambda \cR(\cdot)$ with a conditioning step that maintains the conditioning of $\bSigma_{22}$. This step only changes the realization of the filter $\sfK$, without affecting the objective value.

%\mscomment{to do}\kzcomment{I think this part seems to be a bit underemphasized so far? should we mention this in the Contribution part, when introducing our algorithm (since we are not just doing policy search on the regularized obj)? Also, I guess we do not view it as one of our ``techniques'',  where should we put this part in the Intro section?}
%\jucomment{In the end, conditioning the internal state covariance turned out to be important for ensuring compactness of level sets. Perhaps that could be emphasized here, especially in light of the above theorem which requires compactness?}
%Compact, similarity transformations, 


\begin{comment}
Unfortunately this is not true in general. 
There are a number of 
potential obstacles 
that must be carefully investigated before one may conclude whether or not gradient descent will succeed on these problems.
Some of these are small technicalities.
For instance, in most control problems the loss function is not well-defined (finite) for all policy parameters $\jx\in\R^\jnx$,
and we must restrict our analysis to \emph{stabilizing} policies. 
Other technicalities are more nuanced.
\cref{fact:no_suboptimal_sp} relies on \emph{differentiability} of the functions $\jf(\jx)$ and $\jch(\jn)$.
\jucomment{Check: not that it matters for us, but is the $\hinf$ cost differentiable?}
In addition, \cref{ass:convex_reform_simple} requires that $\jch(\jn) \mapsto \jx$ is surjective.
When $\jx$ parametrizes a transfer function, as is the case for \OE,
the validity of this assumption is complicated by the existence of \emph{similarity transformations} that give (infinitely) many equivalent \emph{realizations} $\jx$ of the same filter. 

Though far from trivial, these technicalities can be resolved by the careful use of slightly more refined mathematical machinery.
In contrast, the greatest obstacle precluding the application of \cref{fact:no_suboptimal_sp} to problems like \OE\
is the assumption that the convex reformulation actually exists (i.e. remains well-defined) at all parameters of interest.  
Consider the \LQG\ cost as a function of the state-space realization of the controller.
This cost function can be made convex via a change of variables [SCHERRER], 
and yet is known to have suboptimal stationary points CITE[LINA].
As we shall see, this apparent contradiction is resolved by the fact that the convexifying change of variables `breaks down' (i.e. is no longer well-defined) at certain parameter values, including those at which suboptimal stationary points arise. 
In this work, for the \OE\ problem, we circumvent this obstacle through the use of non-trivial regularizers
that steer gradient descent away from 
%such 
regions of parameter space
where such `break downs' occur, 
while preserving global optimality of the Kalman filter. 

\jucomment{Do we want to talk about convergence rates here? i.e. give the weak gradient dominance fact, in the style of \cref{fact:no_suboptimal_sp}? My feeling is that it might be a bit too much?}

\begin{enumerate}
\item simple theorem saying we are aware of convex reformulation
\item highlight the major technical hurdles involved in solving the problem
\item targeted for the expect
\end{enumerate}
\end{comment}


\subsection{Related Work}

\paragraph{Solution of the \OE\ problem\ \& Convex reformulation. }

The solution to the \OE\ problem\footnote{\cite{kalman60new} addresses the discrete-time problem, with $\sO=\sC$.} is given by the celebrated \emph{Kalman filter}, as presented in the landmark work of \cite{kalman60new}.
The problem received renewed attention as 
a subproblem used
%one of the two problems solved 
to obtain the solution to \LQG, cf. in particular, the state-space solution of \cite{dgkf89}.
Later, linear matrix inequality (LMI) solutions for \OE\ - 
as well as many other control problems, including $\htwo$, $\hinf$, and mixed $\htwo/\hinf$ synthesis - were developed, concurrently and independently, by \cite{scherer97lmi} and \cite{masubuchi1998lmi}.
The methods were based on convex reformulations of the variety described in \cref{sec:techniques},
and represent non-trivial generalizations of the well-known change of variables used to obtain LMI formulations of static state feedback problems, cf. \cite{thorp1981guaranteed,bernussou1989robust}. 

It has long been appreciated that most cost functions optimized 
during synthesis of controllers and predictors are \emph{nonconvex} in the policy parameters, 
particularly when policies are parametrized in terms of state-space realizations, as in \cref{eq:filter_system}.
As a result, most synthesis procedures were either indirect, reconstructing policies from the 
solutions of Riccati equations (e.g. \cite{dgkf89}) or LMIs (e.g. \cite{scherer97lmi}),
or made use of (model-based) policy parametrizations that rendered the cost function convex, such as the celebrated Youla-Kučera parametrization (a.k.a. $Q$-parametrization), cf. \cite{youla1976parti,youla1976partii,kuvcera1975stability}.
%Only when these aforementioned strategies were inapplicable,
%such as certain distributed control synthesis problems, would one resort to 
%direct search via gradient descent in the space of policy parameters, e.g. \cite{maartensson2009gradient}. 
%The few approaches that did employ 
%Direct search via 
Gradient descent in the space of policy parameters was typically only used
in situations where
%when 
the aforementioned strategies were not applicable, such as certain distributed control synthesis problems, e.g. \cite{maartensson2009gradient}. 

\paragraph{Direct policy search for  control with full state observation.}  Recent years have, however, witnessed a surge of interest in direct policy search, driven perhaps in part by the success of such approaches in reinforcement learning, e.g. \cite{schulman2015trust,schulman2017proximal,openai2020manipulation}. 
Most of this research has focused on problems with perfect state information.
For instance,
\cite{fazel18lqr} establishes global convergence of policy gradient methods on the discrete-time linear quadratic regulator (\LQR) problem,
arguably the simplest continuous state-action optimal control problem.
Subsequent work has sharpened rates \citep{malik2019derivative},
analyzed convergence under more general frameworks 
 \citep{bu2019lqr}, and 
extended the analysis to work in continuous-time  \citep{mohammadi2021convergence}. 


Beyond \LQR,
\cite{zhang20mixed} analyzed global convergence 
of policy search for mixed $\htwo/\hinf$ control and risk-sensitive control. \cite{furieri2020learning} and \cite{li2021distributed} established the  convergence of policy search for certain distributed control problems.  
%objectives (which includes risk sensitive control as a special case).
For discrete state-action (discounted) Markov decision processes (MDPs),
\cite{agarwal2021theory} established convergence rates for a variety of policy gradient methods with both tabular and parametric policies(c.f  \cite{bhandari2019global}).  All of these works considered \emph{static} state-feedback policies, 
%which are sufficient (optimal) the problems studied: 
which are optimal for
their respective problems with full state observation. 

\paragraph{Problems with partial observation.}

Despite their popularity in recent theoretical analysis, problems with perfect state observation are the exception rather than the norm in practice. The key challenge in partial observation is that the optimal policy has to take into account the entire history of observations, which usually yields a {\it dynamic}, rather than static policy. 

For this class of problems, the most  relevant piece of related work is \cite{tang2021analysis}, which studies the optimization landscape of the \LQG\ in continuous time. 
They establish that all stationary points whose corresponding controllers are controllable and observable are globally optimal.
However, they also show (both empirically and via theoretical counterexamples) that gradient descent routinely fails to converge to globally optimal policies; a finding that, as we shall show, remains valid even for the simpler \OE\ problem. 
\cite{fatkhullin2021optimizing} also consider linear quadratic control in the partially observed setting, but restrict their attention to \emph{static} output feedback policies, and provide conditions under which gradient descent converges to (possibly suboptimal) stationary points. 


==> body/regularization.tex <==
Not sure if this is actually true (in general).
\begin{lemma}\label{lem:hot}
Let $f:\real^n\mapsto \real$ be a function such that $\grad f(x)$ exists at $x$.
Then 
\begin{equation*}
\grad_d f(x) \defeq  \lim_{h\rightarrow 0} \frac{f(x + hd) - f(x) }{h} {=} \lim_{h\rightarrow 0} \frac{f(x + hd + \hot) - f(x) }{h}, 
\end{equation*}
where $\hot$ denotes `higher order terms' in $h$, e.g. $\hot = h^2 e + \dots $.
\end{lemma}
\begin{proof}
To-do (if true).
Intuition: the identity should be true for polynomials.
For analytic functions, if we replace $f$ with it's Taylor series expansion, then the identity should hold.
\end{proof}

Now we specialize to the `partially observable control' setting. 
In particular, let $\params=\lbr\cparams\rbr$ denote the parameters of an LTI system.
Consider an objective function $\obj(\params)$ with the following property:
\begin{assumption}\label{ass:minimal_stat_opt}
Let $\bar{\params}$ denote a stationary point of $\obj$, i.e. $\grad \obj(\bar{\params})=0$.
If $\bar{\params}$ corresponds to a minimal realization, then $\bar{\params}$ is a global minimizer of $\obj$. 
\end{assumption}
An example of such a function $\obj$ is the LQG optimal control objective, where $\params=\lbr\cparams\rbr$ denotes a state-space parametrization of the controller.

\emph{Actually, I should think about the definition of $\ccg$, as perhaps there are two possibilities:}
\begin{enumerate}
	\item Let $\ccg(\params)$ denote the controllability Gramian of the system (controller) parametrized by $\params$. 
	\item Let $\ccg(\params)$ denote the steady-state covariance of the state of the controller, in closed-loop with the plant.
\end{enumerate}
The two quantities are different, but both share the property that $\ccg$ will lose rank when $\params$ is not controllable.
The former has the advantage of being computable (exactly) given $\x$ (i.e. does not have to be approximated with data).

Define the regularizer 
\begin{equation}
\regf(\params) = \| \ccg(\params) - \ccg(\params)\inv \|_F^2,
\end{equation}
and the regularized objective 
\begin{equation}
\robj(\params) = \obj(\params) + \regf(\params).
\end{equation}

\begin{lemma}
Let $\stpt{\params}$ denote a stationary point of $\robj$, i.e. $\grad \robj(\stpt{\params})=0$.
Then $\grad \obj(\stpt{\params}) = \grad \regf(\stpt{\params}) = 0$. 
\end{lemma}

\begin{proof}
Equivalently, we are claiming that there exists no point $\stpt{\params}$ such that $\grad \obj(\stpt{\params}) = -\grad \regf(\stpt{\params}) \neq 0$.
%Let us first give the intuition of the proof. 
Suppose we can find a direction $\dir$ (in $\params$-space) such that 
\begin{equation}\label{eq:dir_cond}
\grad_\dir \obj(\spoint) = \grad \obj(\spoint) \cdot \dir =0, \quad \grad_\dir \regf(\spoint) = \grad \regf(\spoint) \cdot \dir \neq 0.
\end{equation}
Then $\grad \robj(\spoint)\cdot\dir = \grad \obj(\spoint) \cdot \dir + \grad \regf(\spoint) \cdot \dir \neq 0$ which contradicts the claim that $\grad \robj(\spoint)=0$.
Hence $\spoint$ cannot be a stationary point. 

So the task now becomes to show that such a $\dir$ satisfying \eqref{eq:dir_cond} always exists, for every $\params$ such that $\grad \regf(\params) \neq 0$. 
(It is sufficient to consider only $\spoint$ such that $\grad\robj(\spoint)=0$, but it turns out we can find such a $\dir$ for all $\params$). 

We will construct such a $\dir$ by considering similarity transformations of $\params$.
In particular, consider matrices of the form
\begin{equation}
T = I + \h \dt, 
\end{equation}
for some scalar $\h$ and matrix $\dt$. 
Let $\simt(\params, T)$ denote similarity transformation of $\params$ using $T$, i.e.,
\begin{equation}
\params' = \lbr \ac',\bc',\cc',\dc'\rbr = \simt(\x,T), \quad \ac'=T\ac T\inv, \ \bc' = T\bc, \ \cc' = \cc T\inv, \ \dc' = \dc.
\end{equation}
For sufficiently small $\h$, we have 
\begin{equation}
T\inv = (I+\h\dt)\inv = I - \h\dt + \h^2 \dt^2 + \dots.
\end{equation}
Therefore, we also have 
\begin{subequations}\label{eq:simt_expansion}
	\begin{align}
	\ac' = T\ac T\inv & = \ac + \h(\dt\ac + \ac \dt) + \h^2\dots \\ 
	\bc' = T\bc &= \bc + \h\dt\bc \\
	\cc' = \cc T\inv & = \cc - \h \cc\dt + \h^2 \dots. 
	\end{align}
\end{subequations}
Looking at the first order approximation of $\params'=\simt(\params,T)$ a natural candidate for such a direction is 
\begin{equation}\label{eq:dir}
\dir=\lbr \dt\ac + \ac \dt, \ \dt\bc, \  -\cc\dt\rbr.
\end{equation}
For convenience, define $\shot(\params,\h,\dt)$ such that \eqref{eq:simt_expansion} can be rewritten as
\begin{equation}\label{eq:shot}
\simt(\params,T) = \params + \h\dir + \shot(\params,\h,\dt).
\end{equation}

Next, we show that with the choice of $\dir$ in \eqref{eq:dir} we 
satisfy the first condition in \eqref{eq:dir_cond}, i.e.
%have 
$\grad_\dir \obj(\params) =0$.
\begin{subequations}
\begin{align}
\grad_\dir \obj(\params) & = \lim_{\h\rightarrow 0} \frac{\obj(\params + \h \dir) - \obj(\params) }{\h} \\
& =  \lim_{\h\rightarrow 0} \frac{\obj(\params + \h \dir + \shot(\params,\h,\dt)) - \obj(\params)}{\h} \label{eq:fproof_1} \\
& = \lim_{\h\rightarrow 0} \frac{\obj(\simt(\params,T)) - \obj(\params)}{\h}  \label{eq:fproof_2} \\
& = \lim_{\h\rightarrow 0} \frac{\obj(\params) - \obj(\params)}{\h}  \\
& = 0,
\end{align}
\end{subequations}
where \eqref{eq:fproof_1} follows from Lemma \ref{lem:hot}, and
\eqref{eq:fproof_2} relies on the fact that $\simt(\params,T) = \params + \h\dir + \shot(\params,\h,\dt)$, cf. \eqref{eq:shot}.
It is important to emphasize that $\grad_\dir \obj(\params) =0$ for $\dir$ defined with \emph{any} $\dt$. 

Next, we show that with $\dir$ as in \eqref{eq:dir} we satisfy the second condition in \eqref{eq:dir_cond}, i.e. $\grad_\dir \regf(\spoint) \neq 0$.
First note that under a similarity transformation $T$ we have 
\begin{equation}
\ccg(\simt(\params,T)) = T\ccg(\params)T\transp. 
\end{equation}
Henceforth, for brevity, let us define $\ccg\defeq\ccg(\params)$. 
Furthermore, note the following identities, easily verified by simple algebra:
\begin{itemize}
	\item $\regf(\params) = \trace ( \ccg^2 + \ccg^{-2} - 2I )$,
	\item $(T\ccg T\transp)\inv = T\invtransp \ccg\inv T\inv$, 
	\item $\regf(\simt(\params,T)) = \trace \left( (\ccg + \h(\dt\ccg+\ccg\dt\transp)  + \hot )^2 +  (\ccg\inv - \h(\dt\transp \ccg\inv +\ccg\inv \dt)  + \hot )^2 - 2I \right)$.
\end{itemize}
Combining these identities gives 
\begin{align}\label{eq:reg_minus_reg}
& \regf(\simt(\params,T))-\regf(\params) = \nonumber \\ 
& \trace \left( \h \left( \ccg(\dt\ccg+\ccg\dt\transp) + (\dt\ccg+\ccg\dt\transp)\ccg \right) - \h\left( \ccg\inv(\dt\transp \ccg\inv +\ccg\inv \dt)  + (\dt\transp \ccg\inv +\ccg\inv \dt)\ccg\inv  \right) + \hot \right).
\end{align}
Our goal is simply to show that there exists \emph{some} direction $\dir$ such that $\grad_\dir \regf(\spoint) \neq 0$.
Recall also that $\grad_\dir \obj(\params) =0$ for $\dir$ defined with \emph{any} $\dt$. 
Factoring $\ccg=UDU\transp$, consider the choice $\dt= UMU\transp$ with diagonal $M$.
Substituting this choice of $\dt$ into \eqref{eq:reg_minus_reg} gives
\begin{align}
 \regf(\simt(\params,T))-\regf(\params)  
 = \trace \ U \left( \h \left( 2DMD + D^2M + MD^2\right) - \h \left( 2D\inv M D\inv + D^{-2}M + MD^{-2}  \right)    \right) U\transp  + \hot. 
\end{align}
With $[D]_{ii} = d_i$ and $[M]_{ii}=m_i$ this reduces to 
\begin{align}\label{eq:reg_sum_form}
\regf(\simt(\params,T))-\regf(\params)  
= 4\h \sum_i m_i \left(  d_i^2 - \frac{1}{d_i^2}  \right) + \hot. 
\end{align}
The quantity $d_i^2-d_i^{-2}=0$ if and only if $d_i=1$.
Therefore, $d_i^2-d_i^{-2}=0$ for all $i$ if and only if $\ccg = I$. 
When $\ccg = I$, we have $\grad\regf(\params) = 0$.
So as long as $\grad\regf(\params)\neq0$, we have $d_i^2-d_i^{-2}\neq0$ for some $i$. 
Then we can make \eqref{eq:reg_sum_form} non-negative by simply choosing $m_i > 0$ if $d_i \geq 1$, and $m_i < 0$ if $0< d_i < 1$.
This gives $\regf(\simt(\params,T))-\regf(\params) = 4\h \epsilon + \hot$, where $\epsilon = \sum_i m_i(d_i^2-d_i^{-2}) > 0$. 

The directional derivative is then given by
\begin{subequations}
\begin{align}
\grad_\dir \regf(\params) & =\lim_{\h\rightarrow 0} \frac{\regf(\params + \h \dir) - \regf(\params) }{\h} \\
& = \lim_{\h\rightarrow 0} \frac{\regf(\params + \h \dir + \shot(\params,\h,\dt)) - \regf(\params) }{\h}  \\
& =  \lim_{\h\rightarrow 0} \frac{\regf(\simt(\params,T)) - \regf(\params) }{\h} \\
&=  \lim_{\h\rightarrow 0} \frac{ 4\h \epsilon + \hot}{\h} \\
&= 4\epsilon > 0.  
\end{align}
\end{subequations} 
\end{proof}


==> body/simulations.tex <==
%!TEX root = ../colt_main.tex

In this subsection we present the results of a number of additional numerical experiments illustrating the performance of \algname.

\paragraph{Random generation of true systems. }
Each experimental trial begins with the random generation of a \emph{true system} of the form \cref{eq:true_system}.
System parameters $\sA,\sC$ are randomly generated using \texttt{Matlab}'s \texttt{rss} function,
with state dimension $\nx = 2$ and output dimension $\ny = 1$. 
The matrix $\sO$ defining the mapping from state to performance output $\po$ is set to $\sO=I$.
The intensity of the system disturbances is randomly generated as $\sW = \tmpW^\top\tmpW$ with each entry of $\tmpW \in\R^{\nx\times\nx}$ sampled from $\calN(0,1)$. 
The intensity of the measurement noise is normalized to $\sV=1$.  
To select suitable systems, we then rejection sample 
%these randomly generated systems 
according to the following criteria:
i) $\sA$ must be strictly stable, and the observability Gramian $\obsv$ corresponding to $(\sA,\sC)$ must satisfy 
$10^{-4} \leq  \lambda_{\min}(\obsv) \leq 10^{-2}$;
ii) $\sW$ must satisfy $\lambda_{\max}(\sW) \leq 5$;
iii)~the optimal cost must satisfy $\Loe(\fparams_\opt) \leq 10^3$. 
The first criterion regulates the observability of the true system, which sets the difficulty of the filtering problem; 
the second ensures that the ratio between the disturbances and measurement noise remains ``reasoanble'';
and the third ensures that the problem instance is not ``pathological'', as determined by excessively high cost of the optimal filter.

\begin{remark}[Choice of $\sO=I$.]
As detailed in \cref{sec:algorithm}, \algname\ makes use of the regularizer $\regexp$, defined in \cref{eq:cL_def},
the computation of which requires access to the true system states $\sx$, as described in \cref{sec:prelim}.
To facilitate a more fair comparison with direct minimization of $\Loe$, we selected $\sO=\eye$ to effectively give the optimizer of $\Loe$ access to the true system states $\sx$ as well. 
As a result, all algorithms compared in this section have access to the same information concerning the true system. 
\end{remark}

\paragraph{Random generation of initial filters. }
Next we randomly generate a filter $\kinit$ from which to initialize gradient descent. 
To do so, we take the optimal (Kalman) filter $\kopt$, and randomly perturb each of the parameters; 
specifically, we set $(\kinit)_i = (\kopt)_i + \delta_i$ with $\delta_i\sim\calN(0,100)$ for the $i$th parameter. 
Before accepting this $\kinit$, we rejection sample based on the following criteria:
i) $\bSigma_{\kinit}$ must satisfy $10^{-5} \leq \sigma_{\min}(\bSigma_{12,\kinit}) \leq 10^{-3}$;
ii) $\bSigma_{\kinit}$ must satisfy $10^{-3} \leq \sigma_{\min}(\bSigma_{22,\kinit}) \leq 1$;
iii) the initial suboptimality must satisfy $\Loe(\kinit) \leq 100 \times \Loe(\kopt)$. 
The first criterion ensures that we do not begin from an initial guess for which the informativity is too low, nor a guess for which it is too high (which makes the search easier).
The second criterion ensures that the initial filter is sufficiently controllable, to avoid initializations that are too close to suboptimal stationary points.
The final criterion ensures that the initial guess is, in all other ways, ``reasonable'', as measured by suboptimality.  

\paragraph{Optimization methods compared. }
Given a randomly generated true system, and random initial filter $\kinit$, we then apply the following three optimization algorithms:
%\jucomment{Will come up with shorthand names later.}
%\begin{enumerate}[i.]
%	\item gradient descent on $\Loe(\fparams)$,
%	\item gradient descent on $\Loe(\fparams)$ with filter state normalization performed before each gradient step, cf. \cref{eq:normalization}
%	\item \algname, as detailed in \cref{alg:our_algorithm}. 
%\end{enumerate}
i) gradient descent on $\Loe(\fparams)$;
ii) gradient descent on $\Loe(\fparams)$ with filter state normalization performed before each gradient step, cf. \cref{eq:recond};
iii) \algname, as detailed in \cref{alg:our_algorithm}, with regularization parameter $\lambda=10^{-4}$. 
See below for further discussion on the selection of $\lambda$.   
All methods are initialized from the same $\kinit$, and make use of the same backtracking line search to select step sizes. 
Moreover, all algorithms have the same termination criteria.
Each algorithm terminates when either:
i) the Frobenius norm of the gradient of the cost function being minimized (either $\Loe$ or $\cL_\lambda$) falls below a tolerance of $10^{-8}$;
ii) the step size selected by the line search falls below a tolerance of $10^{-16}$ for more than three consecutive iterations; or
iii) the number of iterations (gradient descent steps) exceeds $100,000$. 

\paragraph{Results. }
The results of 60 such experimental trials are depicted in \cref{fig:suboptimality}.
It is evident that simple ``unregularized'' gradient descent on $\Loe$ routinely fails to converge to the global optimum, in the allotted number of iterations.
In fact, the median (normalized) suboptimality gap $\frac{\Loe(\fparams) - \Loe(\kopt)}{\Loe(\kopt)}$ exceeds $10^{-4}$,
and only a single trial achieves suboptimality less than $10^{-7}$. 
Loss of informativity in these trials can be seen clearly in \cref{fig:conditioning}.
The addition of the 
filter state reconditioning procedure of \cref{eq:recond} offers only minimal improvement. 
In contrast, \algname\ converges reliably to high-quality solutions that are extremely close to the global optimum; the median normalized suboptimality gap was zero, to numerical precision.  
In fact, for one third of trials, the suboptimality gap was actually \emph{negative} (by very small margins, e.g. $10^{-17}$) indicating that \algname\ has reached the limits of numerical precision with which \texttt{Matlab}'s \texttt{icare} solves Riccati equations (which we use to compute $\kopt$).

%\begin{figure}[H]
%	\centering
%	\subfloat[Normalized suboptimality at the termination of each algorithm.]{
%		\includegraphics[width=7cm]{figures/boxplots_1}} \hspace{1em}
%	\subfloat[Normalized suboptimality as a function of iteration for each algorithm. The lightly shaded region covers the 10th to 90th percentiles, and the darker region covers the 25th to 75th percentiles. ]{
%		\includegraphics[width=8.7cm]{figures/convergence_1}}
%	\caption{Performance of each algorithm as measured by the normalized suboptimality of the output estimation cost, $\frac{\Loe(\fparams) - \Loe(\kopt)}{\Loe(\kopt)}$. 60 trials of the experimental procedure described in \cref{sec:simulations} are plotted.  
%	}
%	\label{fig:suboptimality}
%\end{figure}

\begin{figure}[htbp]
	\floatconts
	{fig:suboptimality}% label for whole figure
	{\caption{ Performance of each algorithm as measured by the normalized suboptimality of the output estimation cost, $\frac{\Loe(\fparams) - \Loe(\kopt)}{\Loe(\kopt)}$. 60 trials of the experimental procedure described in \cref{sec:simulations} are plotted.  
			In (b), the lightly shaded region covers the 10th to 90th percentiles, and the darker region covers the 25th to 75th percentiles.
	}}% caption for whole figure
	{%
		\subfigure[Normalized suboptimality at the termination of each algorithm.]{%
%			\label{fig:peril_no_reg}% label for this sub-figure
			\includegraphics[width=5.75cm]{figures/boxplots_1}
		}
		\qquad % space out the images a bit
		\subfigure[Normalized suboptimality as a function of iteration for each algorithm.]{%
%			\label{fig:peril_ctrb}% label for this sub-figure
			\includegraphics[width=8.25cm]{figures/convergence_1}
		}
	}
\end{figure}

\paragraph{Selection of regularization parameter $\lambda$. }
Performance of \algname\ is in many instances insensitive to the value of $\lambda$ selected.
However, we observed that handful of experimental trails required $\lambda$ to be chosen more judiciously,
in particular, when the spectral properties of $\grad^{~2}\regexp$ differ significantly from those of $\grad^{~2}\Loe$.
Very small stepsizes may be required when $\lambda_{\max}(\grad^{~2}\regexp)$ is very large,
which means the search may make slow progress in updating $\Ck$, as $\regexp$ is independent of $\Ck$.
We have observed good performance in practice by simply ``turning off'' the regularizer (i.e. setting $\lambda=0$)
when the stepsize becomes excessively small (e.g. drops below $10^{-16}$). 



%\begin{figure}[H]
%	\centering
%	\subfloat[Informativity, as measured by $\sigma_{\min}(\jcov_{12})$. ]{
%		\includegraphics[width=7cm]{figures/Sigma_12_1}} \hspace{1em}
%	\subfloat[Conditioning, as measured by $\sigma_{\min}(\jcov_{22})$.  ]{
%		\includegraphics[width=7cm]{figures/Sigma_22_1}}
%	\caption{	
%		Properties of $\jcov$ for the same 60 trials plotted in \cref{fig:suboptimality}. 	
%		The lightly shaded region covers the 10th to 90th percentiles, and the darker region covers the 25th to 75th percentiles. 
%	}
%	\label{fig:conditioning}
%\end{figure}

\begin{figure}[htbp]
	\floatconts
	{fig:conditioning}% label for whole figure
	{\caption{ Properties of $\jcov$ for the same 60 trials plotted in \cref{fig:suboptimality}. 	
					The lightly shaded region covers the 10th to 90th percentiles, and the darker region covers the 25th to 75th percentiles. 
	}}% caption for whole figure
	{%
		\subfigure[Informativity, measured by $\sigma_{\min}(\jcov_{12})$.]{%
			%			\label{fig:peril_no_reg}% label for this sub-figure
			\includegraphics[width=7cm]{figures/Sigma_12_1}
		}
		\qquad % space out the images a bit
		\subfigure[Conditioning, measured by $\sigma_{\min}(\jcov_{22})$.]{%
			%			\label{fig:peril_ctrb}% label for this sub-figure
			\includegraphics[width=7cm]{figures/Sigma_22_1}
		}
	}
\end{figure}



==> body/smoothness.tex <==
%!TEX root = ../main.tex
\newcommand{\Sigx}{\boldsymbol{\Sigma}_{x}}
\newcommand{\Sigxhat}{\boldsymbol{\Sigma}_{\hat{x}}}
\newcommand{\Sigxhatt}{\boldsymbol{\Sigma}_{t,\hat{x}}}
\newcommand{\Sigxhatz}{\boldsymbol{\Sigma}_{0,\hat{x}}}
\newcommand{\Sigxhatx}{\boldsymbol{\Sigma}_{\hat{x}x}}
\newcommand{\matA}{\mathbf{A}}
\newcommand{\matB}{\mathbf{B}}
\newcommand{\matC}{\mathbf{C}}
\newcommand{\calR}{\mathcal{R}}
%\newcommand{\regexp}{\regexp}
\newcommand{\lossregreg}{\cL_{\lambda,\mu}}
\newcommand{\regbal}{\mathcal{R}_{\mathtt{bal}}}


\kzcomment{general comment: @max, we seem to be using $\bSigma_{ij,\sfK}$ and $\bSigma_{\sfK,ij}$ interchangeably in different sections. Update: I changed everything to Macros.}

%Let us describe the parameterization. 

Recall the definition of the limiting covariance matrix 
\$
\bSigma_{\sfK} = \lim_{t \to \infty} \Exp \begin{bmatrix}
	\matx(t) \matx(t)^\top  & \matx(t) \xhatk(t)^\top \\
	\xhatk(t) \matx(t)^\top & \xhatk(t) \xhatk(t)^\top 
\end{bmatrix} =\begin{pmatrix} \Sigonesys & \Sigkonetwo\\
\Sigkonetwo^\top & \Sigktwo
\end{pmatrix} 
\$
which solves the following Lyapunov equation:
\begin{equation}
 \begin{aligned}
  &\Aclk  \Sigk   + \Sigk  \Aclk^\top + \Wclk = 0, \quad \text{where } \Wclk := \begin{bmatrix} \bW_1 & 0\\
0 & \Bk\bW_2\Bk^\top
\end{bmatrix}.  
\end{aligned}
\end{equation} 
Note that $\Sigk$ depends only on $(\Ak,\Bk)$, but not $\Ck$, and that the first $n \times n$ block of $\Sigk$ do not depend on $\sfK$ at all. Also recall the definitions of  $\Zk$ and $\lossreg(\sfK)$\kzcomment{@max:seems that u have missed some $\lambda$ in the previous sections when introducing $\lossreg(\sfK)$. I did not make the edits since I dont have the token there. just a reminder in case i forget.} as 
\begin{align}
\Zk &= \Sigkonetwo\Sigktwo^{-1}\Sigkonetwo^\top\\
\lossreg(\sfK) &= \Loe(\sfK) + \lambda\cdot \regexp(\sfK) = \lim_{t \to \infty} \Exp[\|\po(t) - \fo(t)\|^2] + \lambda\cdot \trace[\Zk^{-1}]. 
\end{align}
Notice from \Cref{eq:llam_simplify} that  \kzcomment{@max: seems that we are missing $\trace$ for the first term in \Cref{eq:llam_simplify}? Also the parenthesis in \Cref{equ:ftil_def_obj}?}
\$
\cL_{\lambda}(\sfK) &=\lim_{t \to \infty} \Exp\left[ \left\|\sO \sx(t) - \Ck \fx(t)\right\|^2 \right] + \lambda\cdot\trace\left[\Zk^{-1}\right] = \trace\Bigg(\begin{bmatrix}
	\sO & -\Ck
\end{bmatrix}  \bSigma_{\sfK} \begin{bmatrix}
	\sO^\top \\ -\Ck^\top
\end{bmatrix}\Bigg)  + \lambda\cdot\trace\left[\matZ(\bSigma_{\sfK})^{-1}\right]. 
\$
In addition, we also define another regularized objective as 
\#\label{equ:new_reg_loss}
\lossregreg(\sfK) &= \Loe(\sfK) + \regexp(\sfK)+\regbal(\sfK) \\
&= \lim_{t \to \infty} \Exp[\|\po(t) - \fo(t)\|^2] + \lambda\cdot\trace[\Zk^{-1}]+\mu\cdot \big\|\Sigktwo - \Sigktwo^{-1}\big\|_{\fro}^2.\notag 
\#

\begin{comment}
XXXXXXXXXXXXXXXXXXXXXXXXXXX
Consider the dynamical system
\$
\dot{x}(t)&=\matA x(t)+w_1(t)\\
\dot{y}(t)&=\matC x(t)+w_2(t),
\$
where $x(t)\in\RR^d$ is the system state, $y(t)\in\RR^m$ is the measured output available for feedback, $w_1(t)\in\RR^d$ and $w_2(t)\in\RR^m$ are white Gaussian noises with intensity matrices  $\bW_1\succ 0$ and $\bW_2 \succ 0$. Hereafter, we will drop the argument $t$ when it is clear in the context. Moreover, consider the filter/observer  
\$
\dot{\hat{x}}&=\matA_K\hat{x}+\matB_K y,
\$
where $\Ak\in\RR^{d\times d}$ and $\Bk\in\RR^{d\times m}$, 
and let $\sfK=(\Ak,\Bk)$. Note that without loss of optimality, we consider a {\it full-order} observer, i.e., the dimension of $\hat{x}$ is the same as that if $x$. \kzcomment{note that in the later proofs, we sometimes use $\bSigma_{\hat{x}x}^{-1}$ directly, which does not make sense without this full-order assumption. }
It is known that the optimal Kalman filter has the following form
\$
\dot{\hat{x}}&=\matA\hat{x}+\bL (y-\matC \hat{x}),
\$
where $\bL=\bP \bC^\top \bW_2^{-1}$ and $\bP$ is the solution to the Riccati equation
\$
\bA\bP+\bP\bA^\top -\bP\bC^\top \bW_2^{-1}\bC\bP +\bW_1=0.
\$
Let $s=(x,~\hat{x})$, we have the closed-loop system
\$
\dot{s}=\underbrace{\begin{bmatrix} \bA & 0\\
\Bk\bC & \Ak\end{bmatrix}}_{\Aclk(\sfK)} s+\underbrace{\begin{bmatrix} \bI & 0\\ 0& \Bk\end{bmatrix}}_{\bB_{cl}(\sfK)}\begin{bmatrix} w_1\\ 
w_2\end{bmatrix}. 
\$
Define the steady-state covariance of $s=(x,~\hat{x})$ as 
\begin{align*}
\Sigk := \begin{bmatrix} \Sigx(\sfK) & \Sigxhatx(\sfK)^\top\\
\Sigxhatx(\sfK) & \Sigktwo\end{bmatrix},
\end{align*}
which solves the following Lyapunov equation
\#\label{equ:bSigma_def}
\begin{bmatrix} \bA & 0\\
\Bk\bC & \Ak\end{bmatrix}\Sigk+\Sigk\begin{bmatrix} \bA & 0\\
\Bk\bC & \Ak\end{bmatrix}^\top +\begin{bmatrix} \bW_1 & 0\\
0 & \Bk\bW_2\Bk^\top \end{bmatrix} =0.
\#

 


Define 
\begin{align*}
R(\sfK):=\|\Sigktwo - \Sigktwo^{-1}\|_{\fro}^2\\
\regexp(\sfK) := \trace\left[\matZ(\Sigk)^{-1}\right],\quad \text{~~~where~~}\matZ(\bSigma) &:= \Sigxhatx^\top \Sigxhat^{-1}\Sigxhatx. 
%G(\bSigma) :=  R(\sfK)+\trace\left[\matZ(\Sigk)^{-1}\right], \quad \text{~~~where~~}\matZ(\bSigma) &:= \Sigxhatx^\top \Sigxhat^{-1}\Sigxhatx.
\end{align*}
Let's start with cost
\begin{align}\label{equ:def_f_lambda}
\lossreg(\sfK)=\lossreg(\matA_K,\matB_K) &:= \trace\left[\matZ(\Sigk)^{-1}\right]+\lambda\cdot R(\sfK),
%=G(\Sigk), 
\end{align}
with $\lambda=1$. 
Throughout this section, we make the following assumption. \kzcomment{I feel like our previous arguments did not make this assumption explicit. Without this, $\bSigma$ will not necessarily be invertible, nor is $\matZ(\Sigk)$? Note that the invertibility of $\bSigma$ does not imply that of $\matZ(\Sigk)$, i.e., we seem to need a stronger assumption on $\sfK$? What we will need to show later (more carefully), is that the  iterates along the policy gradient updates always satisfy the assumption/always guarantees $\bSigma$ and $\matZ(\Sigk)$ are invertible (if we start from such an initialization satisfying the following assumption).}

\kzcomment{I guess we can show this by showing that $\bSigma$ and $\bZ$ are always invertible on the level set of our regularized objective. However, we may still need to justify how can we easily obtain such an initialization satisfying \Cref{assump:regularity}?}

\mscomment{we just can use extended real fomrulations to make$\regexp$ extended real, and infinite where $\bZ$ and $\bSigma$ are rank deficient }

\begin{assumption}\label{assump:regularity}
	Suppose 1) $\sfK=(\Ak,\Bk)$ stabilizes the closed-loop system, i.e., $\Aclk(\sfK)$ is stable; 2) $\big(\Aclk(\sfK),\bB_{cl}(\sfK)\big)$  is controllable; 3) $\matZ(\Sigk)$ is invertible. 
\end{assumption}

Note that under \Cref{assump:regularity}, $\Sigk\succ 0$. Also note that, by Lemma 3.18 in \cite{zhou1996robust}, $\Sigk\succ 0$ in turn implies that $\big(\Aclk(\sfK),\bB_{cl}(\sfK)\big)$ is controllable. Moreover, notice that the invertibility of $\matZ(\Sigk)$ together with the fact that $\Sigxhatx(\sfK)^\top$ is square implies that the latter is also invertible. 
%Suppose $\sfK=(\Ak,\Bk)$ stabilizes the closed-loop system. 
To apply the meta-theorem in \Cref{prop:opt}, we need the following three steps.

XXXXXXXXXXXXXXXXXXXXXXXXXXX
\end{comment}

 
%\paragraph
%\subsection{Step 1: Smoothness of $\lossreg(\sfK)$.}

First, we formalize the gradient and Hessian of  the objectives  $\lossreg(\sfK)$ and $\lossregreg(\sfK)$. To this end, note that 
%$\lossreg(\sfK)$. 
for any stabilizing $\sfK$, the gradient and  the bilinear form of the Hessian of the objectives can be decomposed as those of $\Loe(\sfK)$, $\regexp(\sfK)$, and $\regbal(\sfK)$. We thus deal with them individually. We take  $\Loe(\sfK)$ as an example to show how these quantities are related. Let $\nabla \Loe(\sfK)$ and $\cH_{\Loe,\sfK}(\cdot,\cdot)$ denote the gradient and  the bilinear form of the Hessian of $\Loe(\sfK)$.  For any $\Delta_{\sfK}=(\Delta_{\Ak},\Delta_{\Bk},\Delta_{\Ck})$ with $\Delta_{\Ak}\in\RR^{n\times n}$, $\Delta_{\Bk}\in\RR^{n\times m}$, and, $\Delta_{\Ck}\in\RR^{p\times n}$ we have 
\#\label{equ:taloy_exp}
\Loe(\sfK+\Delta_{\sfK})=\Loe(\sfK)+\trace\Big(\nabla \Loe(\sfK)^\top \Delta_{\sfK}\Big)+\frac{1}{2}\cH_{\Loe,\sfK}(\Delta_{\sfK},\Delta_{\sfK})+o(\|\Delta_{\sfK}\|_F^2). 
\#
The formulas for $\regexp(\sfK)$ and $\regbal(\sfK)$ are similar. 
The following lemma gives closed-forms for these quantities. 

\begin{lemma}\label{lemma:grad_hessian_form}
	For any $\sfK=(\bA_{\sfK},\bB_{\sfK},\Ck)\in\calKexp$, the gradient of the objectives $\lossreg(\sfK)$  and $\lossregreg(\sfK)$ can be decomposed as the gradients of $\Loe(\sfK)$, $\regexp(\sfK)$, and $\regbal(\sfK)$, given by 
	\#
	\nabla \Loe(\sfK)&= 2\begin{bmatrix}
	0 & 0 & -\bO\Sigkonetwo+\Ck \Sigktwo
\end{bmatrix}
+2\begin{bmatrix}
	0 & \bI
\end{bmatrix}\bH_{\sfK}\begin{bmatrix}
	\Sigkonetwo & \Sigonesys\bC^\top & 0 \\ \Sigktwo & \Sigkonetwo^\top\bC^\top+\Bk\bW_2 & 0
\end{bmatrix}
%+2\begin{bmatrix}
%	0 & \bI
%\end{bmatrix}\bH_{\sfK}\begin{bmatrix} 0 & 0 & 0\\
%0 & \Bk\bW_2  & 0 \end{bmatrix}
\\
	\nabla \regexp(\sfK)&=2\begin{bmatrix}
	0 & \bI
\end{bmatrix}\big(\bR_{\sfK}-\bQ_{\sfK}\big)\begin{bmatrix} \Sigkonetwo  & \Sigonesys\bC^\top & 0\\\Sigktwo & \Sigkonetwo^\top\bC^\top +\Bk\bW_2 & 0 \end{bmatrix}\label{equ:grad_reg_exp}\\
	\nabla \regbal(\sfK)&=2\begin{bmatrix}
	0 & \bI 
\end{bmatrix}\big(\bF_{\sfK}-\bG_{\sfK}\big)\begin{bmatrix} \Sigkonetwo  & \Sigonesys\bC^\top & 0\\\Sigktwo & \Sigkonetwo^\top\bC^\top +\Bk\bW_2 & 0 \end{bmatrix}\label{equ:grad_reg_bal}
%	=\begin{bmatrix}
%	\frac{\partial \lossreg(\sfK)}{\partial \Ak} & \frac{\partial \lossreg(\sfK)}{\partial \Bk}
%	\end{bmatrix}
	\#
	where  $\bQ_{\sfK},\bR_{\sfK},\bF_{\sfK},\bG_{\sfK},\bH_{\sfK}$ are solutions to the following Lyapunov equations 
\#
&\Aclk^\top\bQ_{\sfK}+\bQ_{\sfK}\Aclk + \begin{bmatrix}
0 & \Sigkonetwo^{-\top}\Sigktwo \Sigkonetwo^{-1}\Sigkonetwo^{-\top}\\ \Sigkonetwo^{-1}\Sigkonetwo^{-\top}\Sigktwo \Sigkonetwo^{-1} & 0
\end{bmatrix}
=0\notag\\
&\Aclk^\top\bR_{\sfK}+\bR_{\sfK}\Aclk+ \begin{bmatrix}
0 & 0\\ 0 & \Sigkonetwo^{-1}\Sigkonetwo^{-\top}
\end{bmatrix}
%\Big(\bSigma_{\sfK,\Delta_{\sfK}}'(\sfK,\Delta_{\sfK}),\Delta_{\sfK}\Big)
=0\notag\\
&\Aclk^\top \bF_{\sfK}+\bF_{\sfK}\Aclk+2\begin{bmatrix}
	0 & 0\\
	0 & \Sigktwo\end{bmatrix}=0\label{equ:Lyap_F_def}\\
&\Aclk^\top \bG_{\sfK}+\bG_{\sfK}\Aclk+2\begin{bmatrix}
	0 & 0\\
	0 & \Sigktwo^{-3}
\end{bmatrix}=0\label{equ:Lyap_G_def}\\
&\Aclk^\top \bH_{\sfK}+\bH_{\sfK}\Aclk+\begin{bmatrix}
	\bO^\top \\ -\Ck^\top 
\end{bmatrix}\begin{bmatrix}
	\bO & -\Ck
\end{bmatrix}=0.\label{equ:Lyap_H_def}
\#
%and with 
%\#\label{equ:grad_Reg}
%\nabla \regbal(\sfK)=XXXXXX
%\#
 
	Furthermore, the bilinear form of the Hessian of the objectives $\lossreg(\sfK)$  and $\lossregreg(\sfK)$ can be decomposed as that of $\Loe(\sfK)$, $\regexp(\sfK)$, and $\regbal(\sfK)$, 
	given by 
%		is given by $\cH_K(\Delta_{\sfK},\Delta_{\sfK})=\cH_{\regexp,\sfK}(\Delta_{\sfK},\Delta_{\sfK})+\cH_{\regbal,\sfK}(\Delta_{\sfK},\Delta_{\sfK})$, with  
	\#
	&\cH_{\Loe,\sfK}(\Delta_{\sfK},\Delta_{\sfK})=\trace\Bigg(2\begin{bmatrix}
	0 & -\Delta_{\Ck}
\end{bmatrix}\bSigma_{\sfK}\begin{bmatrix}
	0^\top \\ -\Delta_{\Ck}^\top 
\end{bmatrix}+4\begin{bmatrix}
	0 & -\Delta_{\Ck}
\end{bmatrix}\bSigma_{\sfK,\Delta_{\sfK}}'\begin{bmatrix}
	\bO^\top \\ -\Ck^\top 
\end{bmatrix}+\bH_{\sfK}\notag\\
&\qquad\quad\cdot\Bigg(\begin{bmatrix}
	0 \\ \bI
\end{bmatrix}\Delta_{\Ak,\Bk}\begin{bmatrix}
	0 & \bI \\ \bC & 0
\end{bmatrix}\bSigma_{\sfK,\Delta_{\sfK}}'+\bSigma_{\sfK,\Delta_{\sfK}}'\left(\begin{bmatrix}
	0 \\ \bI
\end{bmatrix}\Delta_{\Ak,\Bk}\begin{bmatrix}
	0 & \bI \\ \bC & 0
\end{bmatrix}\right)^\top +\begin{bmatrix} 0 & 0\\
0 & \Delta_{\Bk}\bW_2\Delta_{\Bk}^\top  \end{bmatrix}\Bigg)\Bigg),\label{equ:hess_Loe}\\
	&\cH_{\regexp,\sfK}(\Delta_{\sfK},\Delta_{\sfK})=2\trace\Bigg(\bZ(\Sigk)^{-2}\Big(\begin{bmatrix}
\bI & 0
\end{bmatrix}\bSigma_{\sfK,\Delta_{\sfK}}'\begin{bmatrix}
\bI\\ 0
\end{bmatrix}-\begin{bmatrix}
\bI & -\Sigkonetwo\Sigktwo^{-1}
\end{bmatrix}\bSigma_{\sfK,\Delta_{\sfK}}'\begin{bmatrix}
\bI\\ -\Sigktwo^{-1}\Sigkonetwo^\top
\end{bmatrix}
%+\begin{bmatrix}
%-\bI & \Sigkonetwo\Sigktwo^{-1}
%\end{bmatrix}\bSigma_{\sfK,\Delta_{\sfK}}'\begin{bmatrix}
%\bI\\ 0
%\end{bmatrix}+
\Big)\notag\\
&\quad \cdot \bZ(\Sigk)^{-1}\Big(\begin{bmatrix}
\bI & 0
\end{bmatrix}\bSigma_{\sfK,\Delta_{\sfK}}'\begin{bmatrix}
\bI\\ 0
\end{bmatrix}-\begin{bmatrix}
\bI & -\Sigkonetwo\Sigktwo^{-1}
\end{bmatrix}\bSigma_{\sfK,\Delta_{\sfK}}'\begin{bmatrix}
\bI\\ -\Sigktwo^{-1}\Sigkonetwo^\top
\end{bmatrix}
%+\begin{bmatrix}
%-\bI & \Sigkonetwo\bSigma_{0,22}^{-1}
%\end{bmatrix}\bSigma_{\sfK,\Delta_{\sfK}}'\begin{bmatrix}
%\bI\\ 0
%\end{bmatrix}+
\Big)\Bigg)\notag\\
&\quad-\trace\Bigg(\bS_{\sfK}\cdot\bigg(\begin{bmatrix}
	0 \\ \bI
\end{bmatrix}\Delta_{\Ak,\Bk}\begin{bmatrix}
	0 & \bI \\ \bC & 0
\end{bmatrix}\bSigma_{\sfK,\Delta_{\sfK}}'+\bSigma_{\sfK,\Delta_{\sfK}}'\left(\begin{bmatrix}
	0 \\ \bI
\end{bmatrix}\Delta_{\Ak,\Bk}\begin{bmatrix}
	0 & \bI \\ \bC & 0
\end{bmatrix}\right)^\top +\begin{bmatrix} 0 & 0\\
0 & \Delta_{\Bk}\bW_2\Delta_{\Bk}^\top  \end{bmatrix}\bigg)\Bigg)
%+\begin{bmatrix}
%-\bI & \Sigkonetwo\bSigma_{0,22}^{-1}
%\end{bmatrix}\bSigma_{\sfK,\Delta_{\sfK}}'\begin{bmatrix}
%\bI\\ 0
%\end{bmatrix}+
\notag\\
&\quad
+2\trace\Bigg(\bZ(\Sigk)^{-2}\begin{bmatrix}
\bI & \begin{bmatrix}
 -\bI & \Sigkonetwo \Sigktwo^{-1} 
\end{bmatrix}\bSigma_{\sfK,\Delta_{\sfK}}'
\begin{bmatrix}
0 \\ \Sigktwo^{-1}
\end{bmatrix}
\end{bmatrix}\bSigma_{\sfK,\Delta_{\sfK}}'\begin{bmatrix}
\bI\\ -\Sigktwo^{-1}\Sigkonetwo^\top
\end{bmatrix}\Bigg),\label{equ:hess_reg_exp}\\
&\cH_{\regbal,\sfK}(\Delta_{\sfK},\Delta_{\sfK})=\trace\Bigg(2\begin{bmatrix}
	0 & \bI 
\end{bmatrix}\bSigma_{\sfK,\Delta_{\sfK}}'\begin{bmatrix}
	0 & 0 \\
	0 & \bI
\end{bmatrix}\bSigma_{\sfK,\Delta_{\sfK}}'\begin{bmatrix}
	0 \\ \bI 
\end{bmatrix}+\bE_{\sfK}\cdot\Bigg(\begin{bmatrix}
	0 \\ \bI
\end{bmatrix}\Delta_{\Ak,\Bk}\begin{bmatrix}
	0 & \bI \\ \bC & 0
\end{bmatrix}\bSigma_{\sfK,\Delta_{\sfK}}' \notag\\
&\qquad+\bSigma_{\sfK,\Delta_{\sfK}}'\left(\begin{bmatrix}
	0 \\ \bI
\end{bmatrix}\Delta_{\Ak,\Bk}\begin{bmatrix}
	0 & \bI \\ \bC & 0
\end{bmatrix}\right)^\top+\begin{bmatrix} 0 & 0\\
0 & \Delta_{\Bk}\bW_2\Delta_{\Bk}^\top  \end{bmatrix}\Bigg)+2\bigg(\begin{bmatrix}
	0 & \Sigktwo^{-1} 
\end{bmatrix}\bSigma_{\sfK,\Delta_{\sfK}}'\begin{bmatrix}
	0 \\ \Sigktwo^{-3} 
\end{bmatrix}\notag\\
&\qquad+\begin{bmatrix}
	0 & \Sigktwo^{-2} 
\end{bmatrix}\bSigma_{\sfK,\Delta_{\sfK}}'\begin{bmatrix}
	0 \\ \Sigktwo^{-2} 
\end{bmatrix}+\begin{bmatrix}
	0 & \Sigktwo^{-3} 
\end{bmatrix}\bSigma_{\sfK,\Delta_{\sfK}}'\begin{bmatrix}
	0 \\ \Sigktwo^{-1} 
\end{bmatrix}\bigg)\begin{bmatrix}
	0 & \bI 
\end{bmatrix}\bSigma_{\sfK,\Delta_{\sfK}}'\begin{bmatrix}
	0 \\ \bI 
\end{bmatrix}\Bigg)\label{equ:hess_reg_bal}
%\\
%	&\cH_{\regbal,\sfK}(\Delta_{\Ak,\Bk},\Delta_{\Ak,\Bk})=XXXXX
	\#
	where $\bSigma_{\sfK,\Delta_{\sfK}}',\bS_{\sfK},\bE_{\sfK}$ are solutions to the following Lyapunov equations
	\# 
	&\Aclk\bSigma_{\sfK,\Delta_{\sfK}}'+\bSigma_{\sfK,\Delta_{\sfK}}'\Aclk^\top + \bP_1(\sfK,\Delta_{\sfK})
%\Big(\bSigma_0(\sfK,\Delta_{\sfK}),\Delta_{\sfK}\Big)
=0\label{equ:Sigma_K_DeltaK_prime_def}\\
&\Aclk^\top \bS_{\sfK}+\bS_{\sfK}\Aclk+\begin{bmatrix}
\bI\\ 0
\end{bmatrix}\bZ(\Sigk)^{-2}\begin{bmatrix}
\bI & 0
\end{bmatrix}-\begin{bmatrix}
\bI\\ -\Sigktwo^{-1}\Sigkonetwo^\top
\end{bmatrix}\bZ(\Sigk)^{-2}\begin{bmatrix}
\bI & -\Sigkonetwo\Sigktwo^{-1}
\end{bmatrix}=0,\notag\\
&\Aclk^\top\bE_{\sfK}+\bE_{\sfK}\Aclk+ 2\begin{bmatrix}
	0 \\ \bI 
\end{bmatrix}(\Sigktwo-\Sigktwo^{-3})\begin{bmatrix}
	0 & \bI 
\end{bmatrix}=0\label{equ:E_K_def}
%\\
%&\Aclk^\top\bT(\sfK)+\bT(\sfK)\Aclk+ \begin{bmatrix}
%	\bO^\top \\ -\Ck^\top 
%\end{bmatrix}\begin{bmatrix}
%	\bO & -\Ck
%\end{bmatrix}=0\label{equ:T_K_def}
	\#
	and  
	\#\label{equ:def_P_1}
	\bP_1(\sfK,\Delta_{\sfK})
%\Big(\bSigma_0(\sfK,\Delta_{\sfK}),\Delta_{\sfK}\Big)
:=\begin{bmatrix} 
	0 \\ \bI
\end{bmatrix}\Delta_{\Ak,\Bk}\begin{bmatrix}
	0 & \bI \\ \bC & 0
\end{bmatrix}\Sigk+\Sigk\left(\begin{bmatrix}
	0 \\ \bI
\end{bmatrix}\Delta_{\Ak,\Bk}\begin{bmatrix}
	0 & \bI \\ \bC & 0
\end{bmatrix}\right)^\top +\begin{bmatrix} 0 & 0\\
0 & \Bk\bW_2\Delta_{\Bk}^\top+\Delta_{\Bk}\bW_2\Bk^\top  \end{bmatrix},
	\#
	with $\Delta_{\Ak,\Bk}:=(\Delta_{\Ak},\Delta_{\Bk})$. 
\end{lemma}

%Before proving the lemma, we first introduce the following useful result. 
\begin{proof}[Proof of \Cref{lemma:grad_hessian_form}]


%Recall that $\Delta_{\Ak,\Bk}:=(\Delta_{\Ak},\Delta_{\Bk})$ and  $\Delta_{\sfK}=(\Delta_{\Ak},\Delta_{\Bk},\Delta_{\Ck})$. 
For sufficiently small $t>0$ such that $\sfK+t\cdot\Delta_{\sfK}$ lies in $\calKexp$, we have 
%satisfies \Cref{assump:regularity}, 
%we have by \Cref{equ:bSigma_def} that
\#\label{equ:bSigma_def_delta}
\Bigg(\Aclk+t\begin{bmatrix}
	0 \\ \bI
\end{bmatrix}\Delta_{\Ak,\Bk}\begin{bmatrix}
	0 & \bI \\ \bC & 0
\end{bmatrix}\Bigg)&\bSigma_t(\sfK,\Delta_{\sfK})+\bSigma_t(\sfK,\Delta_{\sfK})\Bigg(\Aclk+t\begin{bmatrix}
	0 \\ \bI
\end{bmatrix}\Delta_{\Ak,\Bk}\begin{bmatrix}
	0 & \bI \\ \bC & 0
\end{bmatrix}\Bigg)^\top \notag\\
&\qquad+\begin{bmatrix} \bW_1 & 0\\
0 & (\Bk+t\Delta_{\Bk})\bW_2(\Bk+t\Delta_{\Bk})^\top \end{bmatrix} =0,
\#
where $\bSigma_t(\sfK,\Delta_{\sfK})$ is the solution to the Lyapunov equation above corresponding to $\sfK+t\cdot\Delta_{\sfK}$. 
By Lemma B.1. in \cite{tang2021analysis}, we know that 
\#\label{equ:taylor_Sigma}
\bSigma_t(\sfK,\Delta_{\sfK})=\bSigma_0(\sfK,\Delta_{\sfK})+t\cdot \bSigma_0'(\sfK,\Delta_{\sfK})+\frac{t^2}{2}\cdot \bSigma_0''(\sfK,\Delta_{\sfK})+o(t^2),
\#
where notice that $\bSigma_0(\sfK,\Delta_{\sfK})=\Sigk$, and 
$\bSigma_0'(\sfK,\Delta_{\sfK})$ and $\bSigma_0''(\sfK,\Delta_{\sfK})$ satisfy
\#
&\Aclk\cdot\bSigma_0'(\sfK,\Delta_{\sfK})+\bSigma_0'(\sfK,\Delta_{\sfK})\cdot\Aclk^\top + \bP_1(\sfK,\Delta_{\sfK})
%\Big(\bSigma_0(\sfK,\Delta_{\sfK}),\Delta_{\sfK}\Big)
=0\label{equ:sigma_1st_prime}\\
&\Aclk\cdot\bSigma_0''(\sfK,\Delta_{\sfK})+\bSigma_0''(\sfK,\Delta_{\sfK})\cdot\Aclk^\top + 2\bP_2(\bSigma_0',\Delta_{\sfK})
%\Big(\bSigma_0'(\sfK,\Delta_{\sfK}),\Delta_{\sfK}\Big)
=0,\label{equ:sigma_2nd_prime}
\#
with $\bP_1(\sfK,\Delta_{\sfK})$ being defined in \Cref{equ:def_P_1}, and 
\$
%&\bP_1(\sfK,\Delta_{\sfK})
%%\Big(\bSigma_0(\sfK,\Delta_{\sfK}),\Delta_{\sfK}\Big)
%:=\begin{bmatrix}
%	0 \\ \bI
%\end{bmatrix}\Delta_{\sfK}\begin{bmatrix}
%	0 & \bI \\ \bC & 0
%\end{bmatrix}\bSigma_0(\sfK,\Delta_{\sfK})+\bSigma_0(\sfK,\Delta_{\sfK})\left(\begin{bmatrix}
%	0 \\ \bI
%\end{bmatrix}\Delta_{\sfK}\begin{bmatrix}
%	0 & \bI \\ \bC & 0
%\end{bmatrix}\right)^\top +\begin{bmatrix} 0 & 0\\
%0 & \Bk\bW_2\Delta_{\Bk}^\top+\Delta_{\Bk}\bW_2\Bk^\top  \end{bmatrix}\\
&\bP_2(\bSigma_0',\Delta_{\sfK})
%\Big(\bSigma_0(\sfK,\Delta_{\sfK}),\Delta_{\sfK}\Big)
:=\begin{bmatrix}
	0 \\ \bI
\end{bmatrix}\Delta_{\Ak,\Bk}\begin{bmatrix}
	0 & \bI \\ \bC & 0
\end{bmatrix}\bSigma_0'(\sfK,\Delta_{\sfK})+\bSigma_0'(\sfK,\Delta_{\sfK})\left(\begin{bmatrix}
	0 \\ \bI
\end{bmatrix}\Delta_{\Ak,\Bk}\begin{bmatrix}
	0 & \bI \\ \bC & 0
\end{bmatrix}\right)^\top +\begin{bmatrix} 0 & 0\\
0 & \Delta_{\Bk}\bW_2\Delta_{\Bk}^\top  \end{bmatrix}.
\$ 
Note that in the statement of the lemma, we use $\bSigma_{\sfK,\Delta_{\sfK}}'$ to denote $\bSigma_0'(\sfK,\Delta_{\sfK})$ for simplicity, defined as the solution  to  \Cref{equ:Sigma_K_DeltaK_prime_def}. 
Also, notice the identities that for an invertible matrix $S(t)$ of function $t$
\#\label{equ:inverse_id}
(S^{-1})'=-S^{-1}S'S^{-1},\qquad (S^{-1})''=(-S^{-1}S'S^{-1})'=2S^{-1}S'S^{-1}S'S^{-1}-S^{-1}S''S^{-1}.
\#
%Moreover, with small enough $t$, $\bSigma_t(\sfK,\Delta_{\sfK})\succ 0$,  we can thus also do Taylor expansion for $\big(\bSigma_t(\sfK,\Delta_{\sfK})\big)^{-1}$:
%\#\label{equ:taylor_Sigma_inv_0}
%\big(\bSigma_t(\sfK,\Delta_{\sfK})\big)^{-1}=\big(\bSigma_0(\sfK,\Delta_{\sfK})\big)^{-1}+t\cdot \Big(\big(\bSigma_0(\sfK,\Delta_{\sfK})\big)^{-1}\Big)'+\frac{t^2}{2}\cdot \Big(\big(\bSigma_0(\sfK,\Delta_{\sfK})\big)^{-1}\Big)''+o(t^2).
%\#
%Notice the identities that for an invertible matrix $S(t)$
%\#\label{equ:inverse_id}
%(S^{-1})'=-S^{-1}S'S^{-1},\qquad (S^{-1})''=(-S^{-1}S'S^{-1})'=2S^{-1}S'S^{-1}S'S^{-1}-S^{-1}S''S^{-1}.
%\#
%\Cref{equ:taylor_Sigma_inv_0} can thus be written as
%\#\label{equ:taylor_Sigma_inv}
%&\big(\bSigma_t(\sfK,\Delta_{\sfK})\big)^{-1}=\big(\bSigma_0(\sfK,\Delta_{\sfK})\big)^{-1}-t\cdot \big(\bSigma_0(\sfK,\Delta_{\sfK})\big)^{-1}\bSigma_0'(\sfK,\Delta_{\sfK})\big(\bSigma_0(\sfK,\Delta_{\sfK})\big)^{-1}\notag\\
%&\quad+\frac{t^2}{2}\cdot \Big[2\big(\bSigma_0(\sfK,\Delta_{\sfK})\big)^{-1}\bSigma_0'(\sfK,\Delta_{\sfK})\big(\bSigma_0(\sfK,\Delta_{\sfK})\big)^{-1}\bSigma_0'(\sfK,\Delta_{\sfK})\big(\bSigma_0(\sfK,\Delta_{\sfK})\big)^{-1}\notag\\
%&\quad-\big(\bSigma_0(\sfK,\Delta_{\sfK})\big)^{-1}\bSigma_0''(\sfK,\Delta_{\sfK})\big(\bSigma_0(\sfK,\Delta_{\sfK})\big)^{-1}\Big]+o(t^2).
%\#




\vspace{5pt}
\paragraph{Results for $\regexp(\sfK)$.} 

For notational convenience, let $\bZ_t=\bZ(\bSigma_t(\sfK,\Delta_{\sfK}))$, $\bSigma_t=\bSigma_t(\sfK,\Delta_{\sfK})$.  Without confusion from the context, we use $\bZ_0'$, $\bZ_0''$, and $(\bZ_0^{-2})''$ to denote $(\bZ_t)'\biggiven_{t=0}$, $(\bZ_t)''\biggiven_{t=0}$, and $(\bZ_t^{-2})''\biggiven_{t=0}$, respectively. We use $\bSigma_{0,ij}$ with $i,j=1,2$ to denote the $(i,j)$-th block of $\bSigma_0(\sfK,\Delta_{\sfK})$, and $\bSigma_{0,ij}'$ to denote the $(i,j)$-th block of $\bSigma_0'(\sfK,\Delta_{\sfK})$.  
Hence, we have
\#
&\regexp(\sfK+t\Delta_{\sfK})=\regexp(\sfK)-t\cdot \trace\Big(\bZ^{-2}_0\cdot\bZ'_0\Big)
%&\qquad
-\frac{t^2}{2}\cdot \trace\Big(\big(\bZ^{-2}_0\big)'\cdot\bZ'_0+\bZ^{-2}_0\cdot\bZ''_0\Big)+o(t^2)\label{equ:taylor_fkal_1}\\
&=\regexp(\sfK)-t\cdot \underbrace{\trace\bigg(\bZ^{-2}_0\cdot\Big(\bSigma_{0,12}'\bSigma_{0,22}^{-1}\bSigma_{0,12}^\top+\bSigma_{0,12}\big(-\bSigma_{0,22}^{-1}\bSigma_{0,22}'\bSigma_{0,22}^{-1}\big)\bSigma_{0,12}^\top+\bSigma_{0,12}\bSigma_{0,22}^{-1}\bSigma_{0,21}'\Big)\bigg)}_{\circled{1}}\notag\\
%&\qquad +\Sigkonetwo(\sfK,\Delta_{\sfK})\big[\big(\bSigma_{0,22}(\sfK,\Delta_{\sfK})\big)^{-1}\big]'\bSigma_{0,21}(\sfK,\Delta_{\sfK})+\Sigkonetwo(\sfK,\Delta_{\sfK})\big(\bSigma_{0,22}(\sfK,\Delta_{\sfK})\big)^{-1}\bSigma_{0,21}'(\sfK,\Delta_{\sfK})\Big)\bigg)\notag\\
&\qquad-\frac{t^2}{2}\cdot \underbrace{\trace\Big(\big(-\bZ^{-2}_0\bZ_0'\bZ_0^{-1}-\bZ^{-1}_0\bZ_0'\bZ_0^{-2}\big)\cdot\bZ'_0+\bZ^{-2}_0\cdot\bZ''_0\Big)}_{\circled{2}}+o(t^2)\label{equ:taylor_fkal_2}
%\trace\left[\matZ(\Sigk)^{-1}\right]
\# 
where \Cref{equ:taylor_fkal_1} follows by $\big(\trace(\bZ^{-1})\big)'=\trace\big(({d\trace(\bZ^{-1})}/{d \bZ})^\top (d\bZ/dt)\big)=-\trace(\bZ^{-2}\bZ')$; \Cref{equ:taylor_fkal_2} uses the identities  in \Cref{equ:inverse_id}. 


Notice the fact that $\bSigma_{0,ij}=\Sigkijof{\sfK}$, and we use $\bSigma_0'$ to denote $\bSigma_0'(\sfK,\Delta_{\sfK})$.  
Hence, for $\circled{1}$, we further have
\#
\circled{1}&=\trace\Bigg(\begin{bmatrix}
0\\ \bI
\end{bmatrix}\Sigktwo^{-1}\Sigkonetwo^\top\bZ^{-2}_0\begin{bmatrix}
	\bI & 0
\end{bmatrix}\bSigma_{0}'-\begin{bmatrix}
0\\ \bI
\end{bmatrix}\Sigktwo^{-1}\Sigkonetwo^\top\bZ_0^{-2}\Sigkonetwo\Sigktwo^{-1}\begin{bmatrix}
0 & \bI
\end{bmatrix}\bSigma_{0}'+\begin{bmatrix}
\bI \\ 0
\end{bmatrix}\bZ_0^{-2}\Sigkonetwo\Sigktwo^{-1}\begin{bmatrix}
0 &  \bI
\end{bmatrix}\bSigma_0'\Bigg)\notag\\
&= 2\trace\Bigg(\begin{bmatrix}
0\\ \bI
\end{bmatrix}\Sigktwo^{-1}\Sigkonetwo^\top\bZ^{-2}_0\begin{bmatrix}
	\bI & 0
\end{bmatrix}\bSigma_{0}'\Bigg)-\trace\Bigg(\begin{bmatrix}
0\\ \bI
\end{bmatrix}\Sigktwo^{-1}\Sigkonetwo^\top\bZ_0^{-2}\Sigkonetwo\Sigktwo^{-1}\begin{bmatrix}
0 & \bI
\end{bmatrix}\bSigma_{0}'
%+\begin{bmatrix}
%\bI \\ 0
%\end{bmatrix}\bZ_0^{-2}\Sigkonetwo\Sigktwo^{-1}\begin{bmatrix}
%0 &  \bI
%\end{bmatrix}\bSigma_0'
\Bigg),
\label{equ:taylor_fkal_3}
\#
where \Cref{equ:taylor_fkal_3} uses the symmetry of the matrices. Since $\bSigma_{0}'$ is the solution to the Lyapunov equation \Cref{equ:sigma_1st_prime}, we then have 
\#
&\circled{1}= \trace\bigg(\bQ_{\sfK}\cdot\bP_1(\sfK,\Delta_{\sfK})\bigg)-\trace\bigg(\bR_{\sfK}\cdot \bP_1(\sfK,\Delta_{\sfK})
\bigg)\notag\\
&=\trace\Bigg(\big(\bQ_{\sfK}-\bR_{\sfK}\big)\cdot\bigg(\begin{bmatrix}
	0 \\ \bI
\end{bmatrix}\Delta_{\Ak,\Bk}\begin{bmatrix}
	0 & \bI \\ \bC & 0
\end{bmatrix}\bSigma_{\sfK}+\bSigma_{\sfK}\left(\begin{bmatrix}
	0 \\ \bI
\end{bmatrix}\Delta_{\Ak,\Bk}\begin{bmatrix}
	0 & \bI \\ \bC & 0
\end{bmatrix}\right)^\top 
%\notag\\
%&\qquad 
+\begin{bmatrix} 0 & 0\\
0 & \Bk\bW_2\Delta_{\Bk}^\top+\Delta_{\Bk}\bW_2\Bk^\top  \end{bmatrix}\bigg)\Bigg)
\label{equ:taylor_fkal_4}\\
&=2\trace\Bigg(\begin{bmatrix}
	 \bI & 0 \\ 0 & \bI \\ 0 & 0
\end{bmatrix}\begin{bmatrix}
	0 & \bI \\ \bC & 0
\end{bmatrix}\bSigma_{\sfK}\big(\bQ_{\sfK}-\bR_{\sfK}\big)\begin{bmatrix}
	0 \\ \bI
\end{bmatrix}\cdot\Delta_{\sfK}
+\begin{bmatrix}
	 \bI & 0 \\ 0 & \bI \\ 0 & 0
\end{bmatrix}\begin{bmatrix} 0 & 0\\
0 & \bW_2\Bk^\top   \end{bmatrix}\cdot\big(\bQ_{\sfK}-\bR_{\sfK}\big)\begin{bmatrix}
	0 \\ \bI
\end{bmatrix}\cdot\Delta_{\sfK}\Bigg)
\label{equ:taylor_fkal_5}
\#
where $\bQ_{\sfK}$ and $\bR_{\sfK}$ are the solutions to the following Lyapunov  equations (which can be further simplified due to the invertibility of $\Sigkonetwo$, as shown in the lemma)
\$
&\Aclk^\top\cdot\bQ_{\sfK}+\bQ_{\sfK}\cdot\Aclk + \begin{bmatrix}
0\\ \bI
\end{bmatrix}\Sigktwo^{-1}\Sigkonetwo^\top\bZ^{-2}_0\begin{bmatrix}
	\bI & 0
\end{bmatrix}+\begin{bmatrix}
\bI \\ 0
\end{bmatrix}\bZ_0^{-2}\Sigkonetwo\Sigktwo^{-1}\begin{bmatrix}
0 &  \bI
\end{bmatrix}
%\Big(\bSigma_0(\sfK,\Delta_{\sfK}),\Delta_{\sfK}\Big)
=0\\
&\Aclk^\top\cdot\bR_{\sfK}+\bR_{\sfK}\cdot\Aclk+ \begin{bmatrix}
0\\ \bI
\end{bmatrix}\Sigktwo^{-1}\Sigkonetwo^\top\bZ_0^{-2}\Sigkonetwo\Sigktwo^{-1}\begin{bmatrix}
0 & \bI
\end{bmatrix}
%\Big(\bSigma_0'(\sfK,\Delta_{\sfK}),\Delta_{\sfK}\Big)
=0,
\$
and \Cref{equ:taylor_fkal_4} is due to the substitution of the definition of $\bP_1(\sfK,\Delta_{\sfK})$, and \Cref{equ:taylor_fkal_5} requires some manipulation. Hence, one can recognize $\nabla \regexp(\sfK)$ by noticing that 
\$
-\circled{1}=\frac{d\regexp(\sfK+t\Delta_{\sfK})}{dt}\Biggiven_{t=0}=\trace\Big(\nabla \regexp(\sfK)^\top \Delta_{\sfK}\Big),
\$
i.e., 
\$
\nabla \regexp(\sfK)&=\Bigg(-2\begin{bmatrix}
	0 & \bI
\end{bmatrix}\big(\bQ_{\sfK}-\bR_{\sfK}\big)\bSigma_{\sfK}\begin{bmatrix}
	0 & \bC^\top \\  \bI & 0
\end{bmatrix}
-2\begin{bmatrix}
	0 & \bI
\end{bmatrix}\big(\bQ_{\sfK}-\bR_{\sfK}\big)\begin{bmatrix} 0 & 0\\
0 & \Bk\bW_2  \end{bmatrix}\Bigg)\cdot\begin{bmatrix}
	 \bI & 0 & 0\\ 0 & \bI  & 0
\end{bmatrix}\\
&=2\begin{bmatrix}
	0 & \bI
\end{bmatrix}\big(\bR_{\sfK}-\bQ_{\sfK}\big)\begin{bmatrix} \Sigkonetwo & \Sigonesys\bC^\top & 0\\\Sigktwo & \Sigkonetwo^\top\bC^\top +\Bk\bW_2 & 0\end{bmatrix}. 
\$
%From the proof, we also observe that
%\#\label{equ:Z_0_prime}
%ddd
%\#

Similarly, for $\circled{2}$ in \Cref{equ:taylor_fkal_2}, we have 
\#\label{equ:hessian_circ_2_1}
&-\circled{2}=\frac{d^2\regexp(\sfK+t\Delta_{\sfK})}{dt^2}\Biggiven_{t=0}
%=
=-2\trace\Big(\bZ^{-2}_0\bZ_0'\bZ_0^{-1}\bZ'_0\Big)+\trace\Big(\bZ^{-2}_0\cdot\bZ''_0\Big)
\#
Note that 
\#\label{equ:hessian_circ_2_2}
&\trace\Big(\bZ^{-2}_0\bZ_0'\bZ_0^{-1}\bZ'_0\Big)=\trace\Big(\bZ^{-2}_0\Big(\bSigma_{0,12}'\Sigktwo^{-1}\Sigkonetwo^\top+\Sigkonetwo\big(-\Sigktwo^{-1}\bSigma_{0,22}'\Sigktwo^{-1}\big)\Sigkonetwo^\top+\Sigkonetwo\Sigktwo^{-1}\bSigma_{0,21}'\Big)\bZ_0^{-1}\bZ'_0\Big)\notag\\
&\quad =\trace\Bigg(\bZ^{-2}_0\Big(\begin{bmatrix}
\bI & 0
\end{bmatrix}\bSigma_{0}'\begin{bmatrix}
0\\ \bI
\end{bmatrix}\Sigktwo^{-1}\Sigkonetwo^\top-\Sigkonetwo\Sigktwo^{-1}\begin{bmatrix}
0 & \bI
\end{bmatrix}\bSigma_{0}'\begin{bmatrix}
0\\ \bI
\end{bmatrix}\Sigktwo^{-1}\Sigkonetwo^\top+\Sigkonetwo\Sigktwo^{-1}\begin{bmatrix}
0 & \bI
\end{bmatrix}\bSigma_{0}'\begin{bmatrix}
\bI\\ 0
\end{bmatrix}\Big)\bZ_0^{-1}\notag\\
&\qquad \cdot \Big(\begin{bmatrix}
\bI & 0
\end{bmatrix}\bSigma_{0}'\begin{bmatrix}
0\\ \bI
\end{bmatrix}\Sigktwo^{-1}\Sigkonetwo^\top-\Sigkonetwo\Sigktwo^{-1}\begin{bmatrix}
0 & \bI
\end{bmatrix}\bSigma_{0}'\begin{bmatrix}
0\\ \bI
\end{bmatrix}\Sigktwo^{-1}\Sigkonetwo^\top+\Sigkonetwo\Sigktwo^{-1}\begin{bmatrix}
0 & \bI
\end{bmatrix}\bSigma_{0}'\begin{bmatrix}
\bI\\ 0
\end{bmatrix}\Big)\Bigg)\notag\\
&\quad =\trace\Bigg(\bZ^{-2}_0\Big(\begin{bmatrix}
\bI & 0
\end{bmatrix}\bSigma_{0}'\begin{bmatrix}
\bI\\ 0
\end{bmatrix}-\begin{bmatrix}
\bI & -\Sigkonetwo\Sigktwo^{-1}
\end{bmatrix}\bSigma_{0}'\begin{bmatrix}
\bI\\ -\Sigktwo^{-1}\Sigkonetwo^\top
\end{bmatrix}
%+\begin{bmatrix}
%-\bI & \Sigkonetwo\Sigktwo^{-1}
%\end{bmatrix}\bSigma_{0}'\begin{bmatrix}
%\bI\\ 0
%\end{bmatrix}+
\Big)\bZ_0^{-1}\notag\\
&\qquad \cdot \Big(\begin{bmatrix}
\bI & 0
\end{bmatrix}\bSigma_{0}'\begin{bmatrix}
\bI\\ 0
\end{bmatrix}-\begin{bmatrix}
\bI & -\Sigkonetwo\Sigktwo^{-1}
\end{bmatrix}\bSigma_{0}'\begin{bmatrix}
\bI\\ -\Sigktwo^{-1}\Sigkonetwo^\top
\end{bmatrix}
%+\begin{bmatrix}
%-\bI & \Sigkonetwo\Sigktwo^{-1}
%\end{bmatrix}\bSigma_{0}'\begin{bmatrix}
%\bI\\ 0
%\end{bmatrix}+
\Big)\Bigg),
\#
and 
\#\label{equ:hessian_circ_2_3}
&\trace\Big(\bZ^{-2}_0\cdot\bZ''_0\Big)=\trace\Bigg(\bZ^{-2}_0\cdot\bigg(\begin{bmatrix}
\bI & 0
\end{bmatrix}\bSigma_{0}'\begin{bmatrix}
\bI\\ 0
\end{bmatrix}-\begin{bmatrix}
\bI & -\Sigkonetwo\Sigktwo^{-1}
\end{bmatrix}\bSigma_{0}'\begin{bmatrix}
\bI\\ -\Sigktwo^{-1}\Sigkonetwo^\top
\end{bmatrix}
%+\begin{bmatrix}
%-\bI & \Sigkonetwo\Sigktwo^{-1}
%\end{bmatrix}\bSigma_{0}'\begin{bmatrix}
%\bI\\ 0
%\end{bmatrix}+
\bigg)'\Bigg)\notag\\
&\quad= \trace\Bigg(\bZ^{-2}_0\cdot\bigg(\begin{bmatrix}
\bI & 0
\end{bmatrix}\bSigma_{0}''\begin{bmatrix}
\bI\\ 0
\end{bmatrix}-\begin{bmatrix}
\bI & -\bSigma_{0,12}'\Sigktwo^{-1}-\Sigkonetwo(\bSigma_{0,22}^{-1})'
\end{bmatrix}\bSigma_{0}'\begin{bmatrix}
\bI\\ -\Sigktwo^{-1}\Sigkonetwo^\top
\end{bmatrix}
%+\begin{bmatrix}
%-\bI & \bSigma_{0,12}\Sigktwo^{-1}
%\end{bmatrix}\bSigma_{0}'\begin{bmatrix}
%\bI\\ 0
%\end{bmatrix}+
\notag\\
&\qquad\quad-\begin{bmatrix}
\bI & -\Sigkonetwo\Sigktwo^{-1}
\end{bmatrix}\bSigma_{0}''\begin{bmatrix}
\bI\\ -\Sigktwo^{-1}\Sigkonetwo^\top
\end{bmatrix}-\begin{bmatrix}
\bI & -\Sigkonetwo\Sigktwo^{-1}
\end{bmatrix}\bSigma_{0}'\begin{bmatrix}
\bI\\ -(\bSigma_{0,22}^{-1})'\Sigkonetwo^\top-\Sigktwo^{-1}\bSigma_{0,21}'
\end{bmatrix}\bigg)\Bigg)\notag\\
&\quad= \trace\Bigg(\bZ^{-2}_0\cdot\bigg(\begin{bmatrix}
\bI & 0
\end{bmatrix}\bSigma_{0}''\begin{bmatrix}
\bI\\ 0
\end{bmatrix}-\begin{bmatrix}
\bI & \begin{bmatrix}
 -\bI & \Sigkonetwo\Sigktwo^{-1} 
\end{bmatrix}\bSigma_0'
\begin{bmatrix}
0 \\ \Sigktwo^{-1}
\end{bmatrix}
\end{bmatrix}\bSigma_{0}'\begin{bmatrix}
\bI\\ -\Sigktwo^{-1}\Sigkonetwo^\top
\end{bmatrix}
%+\begin{bmatrix}
%-\bI & \Sigkonetwo\Sigktwo^{-1}
%\end{bmatrix}\bSigma_{0}'\begin{bmatrix}
%\bI\\ 0
%\end{bmatrix}+
\notag\\
&\qquad\quad-\begin{bmatrix}
\bI & -\Sigkonetwo\Sigktwo^{-1}
\end{bmatrix}\bSigma_{0}''\begin{bmatrix}
\bI\\ -\Sigktwo^{-1}\Sigkonetwo^\top
\end{bmatrix}-\begin{bmatrix}
\bI & -\Sigkonetwo\Sigktwo^{-1}
\end{bmatrix}\bSigma_{0}'\begin{bmatrix}
\bI\\ \begin{bmatrix}
0 & \Sigktwo^{-1}  
\end{bmatrix}
\bSigma_{0}'\begin{bmatrix}
-\bI \\ \Sigktwo^{-1}\Sigkonetwo^\top 
\end{bmatrix}
%-\begin{bmatrix}
%0 & \Sigktwo^{-1} 
%\end{bmatrix}\bSigma_{0}'\begin{bmatrix}
%\bI  \\ 0
%\end{bmatrix}
\end{bmatrix}\bigg)\Bigg)\notag\\
&\quad= \trace\Bigg(\bigg(\begin{bmatrix}
\bI\\ 0
\end{bmatrix}\bZ^{-2}_0\begin{bmatrix}
\bI & 0
\end{bmatrix}-\begin{bmatrix}
\bI\\ -\Sigktwo^{-1}\Sigkonetwo^\top
\end{bmatrix}\bZ_0^{-2}\begin{bmatrix}
\bI & -\Sigkonetwo\Sigktwo^{-1}
\end{bmatrix}\bigg)\cdot\bSigma_{0}''\Bigg)
%+\begin{bmatrix}
%-\bI & \Sigkonetwo\Sigktwo^{-1}
%\end{bmatrix}\bSigma_{0}'\begin{bmatrix}
%\bI\\ 0
%\end{bmatrix}+
\notag\\
&\qquad\quad-2\trace\Bigg(\bZ_0^{-2}\begin{bmatrix}
\bI & \begin{bmatrix}
 -\bI & \Sigkonetwo\Sigktwo^{-1} 
\end{bmatrix}\bSigma_0'
\begin{bmatrix}
0 \\ \Sigktwo^{-1}
\end{bmatrix}
\end{bmatrix}\bSigma_{0}'\begin{bmatrix}
\bI\\ -\Sigktwo^{-1}\Sigkonetwo^\top
\end{bmatrix}\Bigg),
\#
where $\bSigma_{0}''$ denotes $\bSigma_0''(\sfK,\Delta_{\sfK})$, which  solves \Cref{equ:sigma_2nd_prime}, and we use $(\bSigma_{0,22}^{-1})'$ to denote $(\bSigma_{t,22}^{-1})'\biggiven_{t=0}$. Hence,  we further write \Cref{equ:hessian_circ_2_3} as
\#\label{equ:hessian_circ_2_4}
\trace\Big(\bZ^{-2}_0\cdot\bZ''_0\Big)
&=\trace\Bigg(\bS_{\sfK}\cdot\bigg(\begin{bmatrix}
	0 \\ \bI
\end{bmatrix}\Delta_{\Ak,\Bk}\begin{bmatrix}
	0 & \bI \\ \bC & 0
\end{bmatrix}\bSigma_0'+\bSigma_0'\left(\begin{bmatrix}
	0 \\ \bI
\end{bmatrix}\Delta_{\Ak,\Bk}\begin{bmatrix}
	0 & \bI \\ \bC & 0
\end{bmatrix}\right)^\top +\begin{bmatrix} 0 & 0\\
0 & \Delta_{\Bk}\bW_2\Delta_{\Bk}^\top  \end{bmatrix}\bigg)\Bigg)
%+\begin{bmatrix}
%-\bI & \Sigkonetwo\Sigktwo^{-1}
%\end{bmatrix}\bSigma_{0}'\begin{bmatrix}
%\bI\\ 0
%\end{bmatrix}+
\notag\\
&\qquad\quad-2\trace\Bigg(\bZ_0^{-2}\begin{bmatrix}
\bI & \begin{bmatrix}
 -\bI & \Sigkonetwo\Sigktwo^{-1} 
\end{bmatrix}\bSigma_0'
\begin{bmatrix}
0 \\ \Sigktwo^{-1}
\end{bmatrix}
\end{bmatrix}\bSigma_{0}'\begin{bmatrix}
\bI\\ -\Sigktwo^{-1}\Sigkonetwo^\top
\end{bmatrix}\Bigg),
\#
where $\bS_{\sfK}$ is the solution to 
\#\label{equ:hessian_circ_2_5}
\Aclk^\top \bS_{\sfK}+\bS_{\sfK}\Aclk+\begin{bmatrix}
\bI\\ 0
\end{bmatrix}\bZ^{-2}_0\begin{bmatrix}
\bI & 0
\end{bmatrix}-\begin{bmatrix}
\bI\\ -\Sigktwo^{-1}\Sigkonetwo^\top
\end{bmatrix}\bZ_0^{-2}\begin{bmatrix}
\bI & -\Sigkonetwo\Sigktwo^{-1}
\end{bmatrix}=0.
\#
Combining \Cref{equ:hessian_circ_2_1,equ:hessian_circ_2_2,equ:hessian_circ_2_3,equ:hessian_circ_2_4,equ:hessian_circ_2_5} completes the results for $\regexp(\sfK)$. 


\vspace{5pt}
\paragraph{Results for $\regbal(\sfK)$.}
Recall that  $\regbal(\sfK)=\|\Sigktwo - \Sigktwo^{-1}\|_{\fro}^2=\trace(\Sigktwo^2+\Sigktwo^{-2}-2\bI)$. For notational convenience, recall that  $\bSigma_{t,22}=\Sigktwoof{\sfK+t\Delta_{\sfK}}$  and $\bSigma_t=\bSigma_t(\sfK,\Delta_{\sfK})$. 
Note that 
\#
\regbal(\sfK+t\Delta_{\sfK})
%=\regbal(\sfK)+t\cdot \trace\big(2\Sigxhat\cdot\Sigxhat'-2\Sigxhat^{-3}\cdot\Sigxhat'\big)\notag\\
%%&\qquad
%&\qquad\qquad\qquad\qquad+\frac{t^2}{2}\cdot \trace\Big(2\Sigxhat'\Sigxhat'+2\Sigxhat\Sigxhat''-2\big(\Sigxhat^{-3}\big)'\Sigxhat'-2\Sigxhat^{-3}\Sigxhat'\Big)+o(t^2)\\
&=\regbal(\sfK)+t\cdot  \underbrace{\trace\bigg(2\bSigma_{0,22}\bSigma_{0,22}'-2\bSigma_{0,22}^{-3}\bSigma_{0,22}'\bigg)}_{\circled{3}}\notag\\
&\qquad\quad+\frac{t^2}{2}\cdot \underbrace{\trace\Big(2\bSigma_{0,22}'\bSigma_{0,22}'+2\bSigma_{0,22}\bSigma_{0,22}''-2\big(\bSigma_{0,22}^{-3}\big)'\bSigma_{0,22}'-2\bSigma_{0,22}^{-3}\bSigma_{0,22}''\Big)}_{\circled{4}}+o(t^2)\label{equ:taylor_R_1} 
%\trace\left[\matZ(\Sigk)^{-1}\right]
\# 
where \Cref{equ:taylor_R_1} uses the fact that $\big(\trace(\bZ^{-2})\big)'=\trace(-2\bZ^{-3}\bZ')$ for symmetric $\bZ$.  For $\circled{3}$, with the identity   that $\bSigma_{0,22}=\Sigktwo$, we have 
\#
&\circled{3}=\trace\bigg(2\begin{bmatrix}
	0 & \Sigktwo
\end{bmatrix}\bSigma_0'\begin{bmatrix}
	0 \\ \bI
\end{bmatrix}-2\begin{bmatrix}
	0 & \Sigktwo^{-3}
\end{bmatrix}\bSigma_0'\begin{bmatrix}
	0 \\ \bI
\end{bmatrix}\bigg)=\trace\bigg(2\begin{bmatrix}
	0 & 0\\
	0 & \Sigktwo
\end{bmatrix}\bSigma_0'-2\begin{bmatrix}
	0 & 0\\
	0 & \Sigktwo^{-3}
\end{bmatrix}\bSigma_0'\bigg)
\notag\\
&\quad =\trace\bigg(\bF_{\sfK}\cdot\bP_1(\sfK,\Delta_{\sfK})-\bG_{\sfK}\cdot\bP_1(\sfK,\Delta_{\sfK})\bigg),\notag \\
&\quad =2\trace\Bigg(\begin{bmatrix}
\bI & 0\\ 0 & \bI \\0 & 0	
\end{bmatrix}
\begin{bmatrix}
	0 & \bI \\ \bC & 0
\end{bmatrix}\bSigma_{\sfK}\big(\bF_{\sfK}-\bG_{\sfK}\big)\begin{bmatrix}
	0 \\ \bI
\end{bmatrix}\cdot\Delta_{\sfK}
+\begin{bmatrix}
\bI & 0\\ 0 & \bI \\0 & 0	
\end{bmatrix}\begin{bmatrix} 0 & 0\\
0 & \bW_2\Bk^\top   \end{bmatrix}\cdot\big(\bF_{\sfK}-\bG_{\sfK}\big)\begin{bmatrix}
	0 \\ \bI
\end{bmatrix}\cdot\Delta_{\sfK}\Bigg)\notag\\
&\quad =\trace\Big(\nabla \regbal(\sfK)^\top \Delta_{\sfK}\Big),\label{equ:taylor_R_2} 
\#
where $\bF_{\sfK}$ and $\bG_{\sfK}$ are the solutions to the Lyapunov equations \Cref{equ:Lyap_F_def,equ:Lyap_G_def}. The arguments follow similarly from those  in \Cref{equ:taylor_fkal_4,equ:taylor_fkal_5}. This gives the formulation of $\nabla \regbal(\sfK)$ as in the lemma. 

For $\circled{4}$, letting $\big(\bSigma_{0,22}^{-3}\big)'$ denote $\big(\bSigma_{t,22}^{-3}\big)'\biggiven_{t=0}$,  we have 
\#\label{equ:taylor_R_3} 
&\circled{4}=\trace\Bigg(2\begin{bmatrix}
	0 & \bI 
\end{bmatrix}\bSigma_0'\begin{bmatrix}
	0 & 0 \\
	0 & \bI
\end{bmatrix}\bSigma_0'\begin{bmatrix}
	0 \\ \bI 
\end{bmatrix}+2\Sigktwo\begin{bmatrix}
	0 & \bI 
\end{bmatrix}\bSigma_0''\begin{bmatrix}
	0 \\ \bI 
\end{bmatrix}-2\big(\bSigma_{0,22}^{-3}\big)'\bSigma_{0,22}'-2\Sigktwo^{-3}\begin{bmatrix}
	0 & \bI 
\end{bmatrix}\bSigma_0''\begin{bmatrix}
	0 \\ \bI 
\end{bmatrix}\Bigg)\notag\\
&=\trace\Bigg(2\begin{bmatrix}
	0 & \bI 
\end{bmatrix}\bSigma_0'\begin{bmatrix}
	0 & 0 \\
	0 & \bI
\end{bmatrix}\bSigma_0'\begin{bmatrix}
	0 \\ \bI 
\end{bmatrix}+2\Sigktwo\begin{bmatrix}
	0 & \bI 
\end{bmatrix}\bSigma_0''\begin{bmatrix}
	0 \\ \bI 
\end{bmatrix}+2\big(\Sigktwo^{-1}\bSigma_{0,22}'\Sigktwo^{-3}+\Sigktwo^{-2}\bSigma_{0,22}'\Sigktwo^{-2}\notag\\
&\qquad+\Sigktwo^{-3}\bSigma_{0,22}'\Sigktwo^{-1}\big)\bSigma_{0,22}'-2\Sigktwo^{-3}\begin{bmatrix}
	0 & \bI 
\end{bmatrix}\bSigma_0''\begin{bmatrix}
	0 \\ \bI 
\end{bmatrix}\Bigg)\notag\\
&=\trace\Bigg(2\begin{bmatrix}
	0 & \bI 
\end{bmatrix}\bSigma_0'\begin{bmatrix}
	0 & 0 \\
	0 & \bI
\end{bmatrix}\bSigma_0'\begin{bmatrix}
	0 \\ \bI 
\end{bmatrix}+2\begin{bmatrix}
	0 \\ \bI 
\end{bmatrix}(\Sigktwo-\Sigktwo^{-3})\begin{bmatrix}
	0 & \bI 
\end{bmatrix}\bSigma_0''+2\bigg(\Sigktwo^{-1}\begin{bmatrix}
	0 & \bI 
\end{bmatrix}\bSigma_0'\begin{bmatrix}
	0 \\ \bI 
\end{bmatrix}\Sigktwo^{-3}\notag\\
&\qquad +\Sigktwo^{-2}\begin{bmatrix}
	0 & \bI 
\end{bmatrix}\bSigma_0'\begin{bmatrix}
	0 \\ \bI 
\end{bmatrix}\Sigktwo^{-2}+\Sigktwo^{-3}\begin{bmatrix}
	0 & \bI 
\end{bmatrix}\bSigma_0'\begin{bmatrix}
	0 \\ \bI 
\end{bmatrix}\Sigktwo^{-1}\bigg)\begin{bmatrix}
	0 & \bI 
\end{bmatrix}\bSigma_0'\begin{bmatrix}
	0 \\ \bI 
\end{bmatrix}\Bigg)\notag\\
&=\trace\Bigg(2\begin{bmatrix}
	0 & \bI 
\end{bmatrix}\bSigma_0'\begin{bmatrix}
	0 & 0 \\
	0 & \bI
\end{bmatrix}\bSigma_0'\begin{bmatrix}
	0 \\ \bI 
\end{bmatrix}+\bE_{\sfK}\Bigg(\begin{bmatrix}
	0 \\ \bI
\end{bmatrix}\Delta_{\Ak,\Bk}\begin{bmatrix}
	0 & \bI \\ \bC & 0
\end{bmatrix}\bSigma_0'+\bSigma_0'\left(\begin{bmatrix}
	0 \\ \bI
\end{bmatrix}\Delta_{\Ak,\Bk}\begin{bmatrix}
	0 & \bI \\ \bC & 0
\end{bmatrix}\right)^\top +\begin{bmatrix} 0 & 0\\
0 & \Delta_{\Bk}\bW_2\Delta_{\Bk}^\top  \end{bmatrix}\Bigg)\notag\\
&\qquad +2\bigg(\Sigktwo^{-1}\begin{bmatrix}
	0 & \bI 
\end{bmatrix}\bSigma_0'\begin{bmatrix}
	0 \\ \bI 
\end{bmatrix}\Sigktwo^{-3}+\Sigktwo^{-2}\begin{bmatrix}
	0 & \bI 
\end{bmatrix}\bSigma_0'\begin{bmatrix}
	0 \\ \bI 
\end{bmatrix}\Sigktwo^{-2}+\Sigktwo^{-3}\begin{bmatrix}
	0 & \bI 
\end{bmatrix}\bSigma_0'\begin{bmatrix}
	0 \\ \bI 
\end{bmatrix}\Sigktwo^{-1}\bigg)\begin{bmatrix}
	0 & \bI 
\end{bmatrix}\bSigma_0'\begin{bmatrix}
	0 \\ \bI 
\end{bmatrix}\Bigg)
\#
where $\bE_{\sfK}$ is the solution to the Lyapunov equation \Cref{equ:E_K_def}. This completes the results for $\regbal(\sfK)$. 


\vspace{5pt}
\paragraph{Results for $\Loe(\sfK)$.} Recall that $\Loe(\sfK)=\trace\bigg(\begin{bmatrix}
	\sO & -\Ck
\end{bmatrix}  \bSigma_{\sfK} \begin{bmatrix}
	\sO^\top \\ -\Ck^\top
\end{bmatrix}\bigg)$ and that $\bSigma_t=\bSigma_t(\sfK,\Delta_{\sfK})$. Hence, we have 
\small
\#
&\Loe(\sfK+t\Delta_{\sfK})
%=\regbal(\sfK)+t\cdot \trace\big(2\Sigxhat\cdot\Sigxhat'-2\Sigxhat^{-3}\cdot\Sigxhat'\big)\notag\\
%%&\qquad
%&\qquad\qquad\qquad\qquad+\frac{t^2}{2}\cdot \trace\Big(2\Sigxhat'\Sigxhat'+2\Sigxhat\Sigxhat''-2\big(\Sigxhat^{-3}\big)'\Sigxhat'-2\Sigxhat^{-3}\Sigxhat'\Big)+o(t^2)\\
=\Loe(\sfK)+t\cdot  \underbrace{\trace\bigg(2\begin{bmatrix}
	0 & -\Delta_{\Ck}
\end{bmatrix}\bSigma_0\begin{bmatrix}
	\bO^\top \\ -\Ck^\top 
\end{bmatrix}+\begin{bmatrix}
	\bO & -\Ck
\end{bmatrix}\bSigma_{0}'\begin{bmatrix}
	\bO^\top \\ -\Ck^\top 
\end{bmatrix}\bigg)}_{\circled{5}}+o(t^2)\label{equ:taylor_Loe_1}\\
&\quad+\frac{t^2}{2}\cdot \underbrace{
%\begin{aligned}
\trace\Bigg(2\begin{bmatrix}
	0 & -\Delta_{\Ck}
\end{bmatrix}\bSigma_0\begin{bmatrix}
	0^\top \\ -\Delta_{\Ck}^\top 
\end{bmatrix}+2\begin{bmatrix}
	0 & -\Delta_{\Ck}
\end{bmatrix}\bSigma_0'\begin{bmatrix}
	\bO^\top \\ -\Ck^\top 
\end{bmatrix}+\begin{bmatrix}
	\bO & -\Ck
\end{bmatrix}\bSigma_{0}''\begin{bmatrix}
	\bO^\top \\ -\Ck^\top 
\end{bmatrix}+2\begin{bmatrix}
	0 & -\Delta_{\Ck}
\end{bmatrix}\bSigma_{0}'\begin{bmatrix}
	\bO^\top \\ -\Ck^\top 
\end{bmatrix}\Bigg)
%\end{aligned}
}_{\circled{6}}.\notag 
%\trace\left[\matZ(\Sigk)^{-1}\right]
\# 
\normalsize
Note that $\bSigma_0=\bSigma_{\sfK}$. 
For \circled{5}, we thus have 
\small
\#
&\circled{5}
%=\trace\bigg(2\begin{bmatrix}
%	0 & -\Delta_{\Ck}
%\end{bmatrix}\bSigma_0\begin{bmatrix}
%	\bO^\top \\ -\Ck^\top 
%\end{bmatrix}+\begin{bmatrix}
%	\bO & -\Ck
%\end{bmatrix}\bSigma_{0}'\begin{bmatrix}
%	\bO^\top \\ -\Ck^\top 
%\end{bmatrix}\bigg)\notag\\
%&\quad 
=\trace\bigg(2\Delta_{\sfK}\begin{bmatrix}
	0 & 0\\0 & 0\\0 & -\bI
\end{bmatrix}\bSigma_{\sfK}\begin{bmatrix}
	\bO^\top \\ -\Ck^\top 
\end{bmatrix}+\begin{bmatrix}
	\bO^\top \\ -\Ck^\top 
\end{bmatrix}\begin{bmatrix}
	\bO & -\Ck
\end{bmatrix}\bSigma_{0}'\bigg)= \trace\bigg(2\begin{bmatrix}
	0 & 0\\0 & 0\\0 & -\bI
\end{bmatrix}\bSigma_{\sfK}\begin{bmatrix}
	\bO^\top \\ -\Ck^\top 
\end{bmatrix}\cdot \Delta_{\sfK}+\bH_{\sfK}\cdot\bP_1(\sfK,\Delta_{\sfK})\bigg)\notag\\
&\quad=2\trace\Bigg(\begin{bmatrix}
	0 & 0\\0 & 0\\0 & -\bI
\end{bmatrix}\bSigma_{\sfK}\begin{bmatrix}
	\bO^\top \\ -\Ck^\top 
\end{bmatrix}\cdot \Delta_{\sfK}+\begin{bmatrix}
\bI & 0\\ 0 & \bI \\0 & 0	
\end{bmatrix}
\begin{bmatrix}
	0 & \bI \\ \bC & 0
\end{bmatrix}\bSigma_{\sfK} \bH_{\sfK} \begin{bmatrix}
	0 \\ \bI
\end{bmatrix}\cdot\Delta_{\sfK}
+\begin{bmatrix}
\bI & 0\\ 0 & \bI \\0 & 0	
\end{bmatrix}\begin{bmatrix} 0 & 0\\
0 & \bW_2\Bk^\top   \end{bmatrix}\bH_{\sfK}\begin{bmatrix}
	0 \\ \bI
\end{bmatrix}\cdot\Delta_{\sfK}\Bigg)\notag\\
&\quad =\trace\Big(\nabla \Loe(\sfK)^\top \Delta_{\sfK}\Big),\label{equ:taylor_Loe_2} 
\#
\normalsize
where $\bH_{\sfK}$ is the solution to the Lyapunov equation  \Cref{equ:Lyap_H_def}. The arguments follow similarly from those  in \Cref{equ:taylor_fkal_4,equ:taylor_fkal_5}. This gives the formulation of $\nabla \Loe(\sfK)$ as in the lemma after some simplification. 

Moreover, for $\circled{6}$ we have
\#\label{equ:taylor_Loe_3} 
&\circled{6}=
\trace\Bigg(2\begin{bmatrix}
	0 & -\Delta_{\Ck}
\end{bmatrix}\bSigma_{\sfK}\begin{bmatrix}
	0^\top \\ -\Delta_{\Ck}^\top 
\end{bmatrix}+4\begin{bmatrix}
	0 & -\Delta_{\Ck}
\end{bmatrix}\bSigma_0'\begin{bmatrix}
	\bO^\top \\ -\Ck^\top 
\end{bmatrix}+\begin{bmatrix}
	\bO^\top \\ -\Ck^\top 
\end{bmatrix}\begin{bmatrix}
	\bO & -\Ck
\end{bmatrix}\bSigma_{0}''\Bigg)\notag\\
&\quad =\trace\Bigg(2\begin{bmatrix}
	0 & -\Delta_{\Ck}
\end{bmatrix}\bSigma_{\sfK}\begin{bmatrix}
	0^\top \\ -\Delta_{\Ck}^\top 
\end{bmatrix}+4\begin{bmatrix}
	0 & -\Delta_{\Ck}
\end{bmatrix}\bSigma_0'\begin{bmatrix}
	\bO^\top \\ -\Ck^\top 
\end{bmatrix}+\bH_{\sfK}\notag\\
&\qquad\quad\cdot\Bigg(\begin{bmatrix}
	0 \\ \bI
\end{bmatrix}\Delta_{\Ak,\Bk}\begin{bmatrix}
	0 & \bI \\ \bC & 0
\end{bmatrix}\bSigma_0'+\bSigma_0'\left(\begin{bmatrix}
	0 \\ \bI
\end{bmatrix}\Delta_{\Ak,\Bk}\begin{bmatrix}
	0 & \bI \\ \bC & 0
\end{bmatrix}\right)^\top +\begin{bmatrix} 0 & 0\\
0 & \Delta_{\Bk}\bW_2\Delta_{\Bk}^\top  \end{bmatrix}\Bigg)\Bigg)
\#
where $\bH_{\sfK}$ is the solution to the Lyapunov equation \Cref{equ:Lyap_H_def}. This completes the results for $\Loe(\sfK)$. \end{proof}


The smoothness follows by \kzcomment{note that we will need to show that $\Ak$, $\Bk$  and $\Ck$ are also bounded in the level sets (so are $\Sigk,\Sigk^{-1},\bZ(\Sigk)^{-1}$).}
\$
&\|\cH_{\Loe,\sfK}+\lambda\cH_{\regexp,\sfK}+\mu\cH_{\regbal,\sfK}\|
\leq \sup\limits_{\|\Delta_{\sfK}\|_{\fro}= 1}\big|\cH_{\Loe,\sfK}(\Delta_{\sfK},\Delta_{\sfK})+\lambda\cH_{\regexp,\sfK}(\Delta_{\sfK},\Delta_{\sfK})+\mu\cH_{\regbal,\sfK}(\Delta_{\sfK},\Delta_{\sfK})\big|\\
&\quad\leq \sup\limits_{\|\Delta_{\sfK}\|_{\fro}= 1}|\cH_{\Loe,\sfK}(\Delta_{\sfK},\Delta_{\sfK})|+\lambda\cdot\sup\limits_{\|\Delta_{\sfK}\|_{\fro}= 1}|\cH_{\regexp,\sfK}(\Delta_{\sfK},\Delta_{\sfK})|+\mu\cdot\sup\limits_{\|\Delta_{\sfK}\|_{\fro}= 1}|\cH_{\regbal,\sfK}(\Delta_{\sfK},\Delta_{\sfK})|\\
&\quad\leq \poly_{\op}\left(\bA,\bC,\Sigk,\Sigk^{-1},\Ak,\Bk,\Ck,               \bZ(\Sigk)^{-1}\right).
\$
 


%For any matrix $\bM,\bN$, we have 
%\#\label{equ:hessian_circ_2_2}
%\trace\Big(\bM\bZ_0'\bN\bZ_0'\Big)
%\#


%Now we formally state one intermediate result used in the proof. 
%
%\begin{lemma}[Lemma B.1. in \cite{tang2021analysis}]\label{lemma:derivative_lemma}
%	Let $M:(-\delta,\delta)\to \RR^{k\times k}$ and $G:(-\delta,\delta)\to \RR^{k\times k}$ with   $G(t)$ being symmetric are two indefinitely differentiable matrix-valued functions for some $\delta>0$. Suppose $M(t)$ is Hurwitz for all $t\in(-\delta,\delta)$. Let $X(t)$ be the solution to the Lyapunov equation 
%	\$
%	M(t)X(t)+X(t)M(t)^\top +G(t)=0.
%	\$
%	Then, $X(t)$ is indefinitely differentiable over $t\in(-\delta,\delta)$, and its $j$-th order derivative at $t=0$, denoted by $X^{(j)}(0)$,  is the solution to the following Lyapunov equation
%	\$
%	M(0)X^{(j)}(0)+X^{(j)}(0)M(0)^\top +\Bigg(\sum_{i=1}^j\frac{j!}{i!(j-i)!}\Big(M^{(i)}(0)X^{(j-i)}(0)+X^{(j-i)}(0)M^{(i)}(0)^\top \Big)+G^{(j)}(0)\Bigg)=0.
%	\$
%%	Furthermore, if the solution $X(t)$ is invertible for $t$ in the neighborhood of $0$, letting  $X^{-(j)}(0)$ denote the $j$-th order derivative of $X^{-1}(t)$, then it satisfies the following  equation 
%%	\$
%%	M(0)X^{(j)}(0)+X^{(j)}(0)M(0)^\top +\Bigg(\sum_{i=1}^j\frac{j!}{i!(j-i)!}\Big(M^{(i)}(0)X^{(j-i)}(0)+X^{(j-i)}(0)M^{(i)}(0)^\top \Big)+G^{(j)}(0)\Bigg)=0.
%%	\$
%\end{lemma}



%\kzcomment{TO DO. Note that only showing the boundedness of $\sfK$ is not sufficient, since we need some quantitative bounds. Bounding Hessian directly?}
%\begin{align*}
%\regexp(\sfK) := \trace\left[\matZ(\Sigk)^{-1}\right]
%\end{align*}



==> preamble/reg_macros.tex <==
\newcommand{\lbr}{\lbrace}
\newcommand{\rbr}{\rbrace}

\newcommand{\ac}{{A_c}}
\newcommand{\bc}{{B_c}}
\newcommand{\cc}{{C_c}}
\newcommand{\dc}{{D_c}}

\newcommand{\cparams}{\ac,\bc,\cc,\dc}
\newcommand{\lmiparams}{X,Y,K,L,M,N}

%\newcommand{\transp}{^{\top}}
\newcommand{\invtransp}{^{-\top}}
\newcommand{\inv}{^{-1}}



\newcommand{\params}{\x}
\newcommand{\obj}{F}
\newcommand{\regf}{R}
\newcommand{\ccg}{\Sigma}
\newcommand{\robj}{G}

%\newcommand{\h}{h}
\newcommand{\dt}{\bar{T}}

\newcommand{\simt}{\mathcal{S}}
\newcommand{\shot}{\mathcal{S}_{\textup{hot}}}

\newcommand{\stpt}[1]{\bar{#1}}

\newcommand{\spoint}{\stpt{\params}}

%\newcommand{\xcl}{\mathcal{X}}
%
%\newcommand{\x}{\mathbf{x}}
%\newcommand{\y}{\mathbf{y}}
\newcommand{\bnu}{\boldsymbol{\nu}}
\newcommand{\ytmp}{\bnu}

\newcommand{\dir}{\mathbf{d}}

\newcommand{\xc}{\bar{x}}

\newcommand{\miniheading}[1]{
	{\vspace{0.5em}
		\parindent0pt 
		\textbf{#1} \\
	}
}

\newcommand{\hot}{\textup{h.o.t}}
